An Aggregation Technique For Large-Scale PEPA Models With Non-Uniform Populations

Performance analysis based on modelling consists of two major steps: model construction and model analysis. Formal modelling techniques significantly aid model construction but can exacerbate model analysis. In particular, here we consider the analysis of large-scale systems which consist of one or more entities replicated many times to form large populations. The replication of entities in such models can cause their state spaces to grow exponentially to the extent that their exact stochastic analysis becomes computationally expensive or even infeasible. In this paper, we propose a new approximate aggregation algorithm for a class of large-scale PEPA models. For a given model, the method quickly checks if it satisfies a syntactic condition, indicating that the model may be solved approximately with high accuracy. If so, an aggregated CTMC is generated directly from the model description. This CTMC can be used for efficient derivation of an approximate marginal probability distribution over some of the model's populations. In the context of a large-scale client-server system, we demonstrate the usefulness of our method.

==> AggregationCondition/aggregationCondition.tex <==
\section{Aggregation and its Condition}
\label{condition}
\subsection{Syntactic Condition}
We consider a sub-class of large-scale PEPA models where the populations of different sequential components have significantly different sizes; i.e. models in which the groups sizes are not uniform. 
It is the modeller's task to decide for every group in a model, whether it constitutes a large group or a small one. 
The modeller introduces a threshold value $\Theta_{\mo{M}}$. Using this, any group $H_i \in \group{M}$ is considered to be small if $\sum_{y=1}^{N_{C_x}} \xi_{i,y} \leq \Theta_{\mo{M}}$; assuming that sub-vector $\boldsymbol\xi_i$ captures the state of the instances in group $H_i$ and $sc(H_i)=C_x$. Conversely, $H_i$ is considered as large if $\sum_{y=1}^{N_{C_x}} \xi_{i,y} > \Theta_{\mo{M}}$.

For a grouped PEPA model $\mo{M}$, let $\smgroup{M}$ denote the set of small groups in $\mo{M}$. Formally, $\smgroup{M} = \{H^{s}_1,H^{s}_2 \ldots, H^{s}_i, \ldots \}$ is the subset of labels in $\group{M}$ where for each $H^{s}_i$, \mbox{$\sum_{y=1}^{N_{C_x}} \xi_{i,y} \leq \Theta_{\mo{M}}$, $C_x = sc(H^{s}_i)$}. 
The model is assumed to have $N^{s}_{\mo{M}}$ small groups.
Similarly, let $\lagroup{M} = \{H^{l}_1,H^{l}_2 \ldots, H^{l}_i, \ldots \}$ denote the set of group labels in $\group{M}$ where for each $H^{l}_{i}$, the respective group is considered to contain a large number of $sc(H^{l}_{i})$ instances.
This characterisation of the groups induces a partition on set $\group{M}$, $\group{M} = \smgroup{M}\  \cup \lagroup{M} $.
Moreover, it will divide $\mathbb{M}$'s state vector into two sections; the state variables (counters) which are related to the groups in $\smgroup{M}$ and the ones related to the groups in $\lagroup{M}$. 
Without loss of generality, the model's complete state vector can be written as $\langle \boldsymbol\xi_{s},\boldsymbol\xi_{l}\rangle$ where $\boldsymbol\xi_{s}$ is related to the model\rq{}s small groups and  $\boldsymbol\xi_{l}$ to the model\rq{}s large groups. 

As $\mathbb{M}$ is assumed to be a large-scale model, its complete CTMC is very large and its construction and analysis requires access to a vast storage facility and powerful computation resources. Additionally, running experiments on the model, such as observing how changing the model's parameters affects its behaviour for a given parameter space, would be infeasible as the analysis of each case consumes a long time. 

We will show that, if the model falls in the above sub-class and satisfies the following condition, then, we can make an \emph{approximate} state space aggregation which results in an aggregated CTMC for the model. Moreover, we illustrate that this step enables us to efficiently estimate a marginal probability distribution over the model's small groups with a high accuracy. The computational cost of finding such a distribution by using the aggregate CTMC is orders of magnitude smaller than that when it gets calculated through the analysis of the original CTMC. 
%Checking the probability of an event which focuses on the configuration of all state counters would entails the construction of the underlying CTMC and solving it. Due to the size of the state space, this possibility is out of question. In this paper, our claim is that when the following condition is respected, then the marginal probability distribution which focus on the configuration of the counters associated to the component type in $P_D$ can be efficiently found without solving the model's underlying CTMC. 
\begin{condition}
\label{aggregationCondition}
{\bf Syntactic Aggregation Condition} For any shared activity, synchronised between one or more large groups and one or more small group, the rate of the shared activity, should be completely decided by the small groups.
Formally, 
\begin{multline*}
  \forall\  H^{l}\ \in\ \lagroup{M} \ \ ,\ \  \forall\ \alpha\  \in\  \einterface{M}{H} \\
 [\ \   (\ \coop{M}{H^{l}}{\alpha}\ \cap\ \smgroup{M} \ ) \not= \emptyset  \implies \\
 \ \ \ \ \ \ \ \forall\ C_{x,y}\  \in\ ds^{*}(H^{l})\ ,\ \exists\  \omega \in \mathbb{N}\ , \ \ r_{\alpha}(C_{x,y}) = \omega \top \ ]
\end{multline*}
\end{condition}
%the intuition behind the condition.
Intuitively, the condition expresses that in the context of any synchronization, which takes place on a shared activity of type $\alpha$, if both small and large groups are involved, then all instances of sequential processes in the relevant large groups are defined to undertake  $\alpha$ activities passively. 
As an example, take the client-server model where the behaviour of the clients is replaced with the following: 
\begin{eqnarray*}
C_{think} & \rmdef & (think, r_t).C_{req}\  \\
C_{req} & \rmdef & (req, \top).C_{think}\
\end{eqnarray*}
The $Clients$, being considered as a large group, and $Servers$, which are regarded as a small one, synchronise on the activity of type $req$ and the clients undertake the activity with a passive rate. 
Therefore, for this model, the aggregation is possible. We will see that this property implies that in any state of the system, the rate observed for an activity of type $req$ depends on the configuration of the servers only and is independent of the clients\rq{} configuration.

\subsection{The CTMC Structure}
\label{sec:ctmcstructure}
The CTMC of a large-scale PEPA model with small groups which satisfies the Condition \ref{aggregationCondition} exhibits important structural properties which can be exploited in order to build an aggregated CTMC. 
In this section, these properties are introduced and then illustrated in the CTMC of a client-server model when initialised with two servers and two clients and assuming that the clients take part in the $req$ activity passively. 
\begin{figure*}[]
\centering
\includegraphics[ width = 1.0\textwidth, height=0.8\textheight]{./graphs/ClientServerModelWithBreakdown2Servers2Clients}
\caption{CTMC of the client-server system initialised with two servers and two clients. \label{fig:fullstatesapce}}
\end{figure*}

Given that the model's groups are partitioned according to being small or large, one can categorise each transition depending on whether it changes the state of some small groups only, the state of some large groups only or simultaneously, the state of some small and large ones. 
For a group $H$, $\actions{H}$ is the set of action types enabled by $H$ and $\actions{H}-\interface{M}{H}$ is the set of action types not offered in $H$\rq{}s interface; i.e. the action types related to the individual activities the instances in $H$ undertake. 
As the first case, assume that $H\in\lagroup{M}$. For this group, we define $\actionsLargeGroup{H}$, the set of action types instances in $H$ support either individually or in cooperation with other large groups.
\begin{multline}
\actionsLargeGroup{H} = \left\{\ \alpha \mid\ \left[\  \alpha \in\  (\ \actions{H}-\interface{M}{H}\ ) \ \right]\right.\ \vee \\
\left. \left[\ \alpha\  \in\  \interface{M}{H} \ \wedge\ (\ \coop{M}{H}{\alpha} \cap \smgroup{M}\ ) = \emptyset \ \vphantom{\actions{H}}\right]\  \right\}
\end{multline}

Using $\actionsLargeGroup{H}$, we can define $\actionsLargeGroup{\mo{M}}$ to denote the set of action types which are related to the dynamics of the large groups only and are not shared with any small ones. 
\[\actionsLargeModel{M} = \bigcup_{H \in \lagroup{M}}^{} \actionsLarge{H}.\]

As the second case, assume that $H\in\smgroup{M}$. Here, we can calculate $\actionsSmallGroup{H}$, representing the set of action types which is enabled by $H$, but not shared with any large group. Note that this set might include the action types instances in $H$ share with instances in other small groups, if such action types exist. 
\begin{multline}
\actionsSmallGroup{H} = \left\{\ \alpha \mid\ \left[\  \alpha \in\  (\ \actions{H}-\interface{M}{H}\ ) \ \right]\right.\ \vee \\
\left. \left[\ \alpha\  \in\  \interface{M}{H} \ \wedge\ (\ \coop{M}{H}{\alpha} \cap \lagroup{M}\ ) = \emptyset \ \vphantom{\actions{H}}\right]\  \right\}
\end{multline}

Using $\actionsSmallGroup{H}$, for model $\mo{M}$, we can calculate $\actionsSmallModel{M}$ which represents the action types in which the large groups do not participate. 
\[\actionsSmallModel{M} = \bigcup_{H \in \smgroup{M}}^{} \actionsSmallGroup{H}.\]

$\mo{M}$ might contain some action types which are shared between the small and large groups. For $H\in\smgroup{M}$, let us define $\actionsSmallLargeGroup{H}$ to represent the set of action types shared between instances of $H$ and instances of one or more large groups. 
\[\actionsSmallLargeModel{M} = \{\ \alpha\ \mid\ \alpha\ \in\ \interface{M}{H} \ \wedge\ (\ \coop{M}{H}{\alpha}\ \cap\ \lagroup{M}\ )\not=\emptyset\ \}\]
Therefore, for model $\mo{M}$, the set of action types in which both small and large groups participate is: 
\[\actionsSmallLargeModel{M} = \bigcup_{H\in\smgroup{M}}^{}\ \actionsSmallLargeGroup{H} .\]
These categorisation of the action types is used when expressing the structural properties of a model which satisfies Condition \ref{aggregationCondition}.

\begin{exmp}
For the client-server system shown in Model \ref{model1}: 
\begin{eqnarray*}
\actionsLargeModel{CS} &=& \{think\} \\
\actionsSmallModel{CS} &=& \{log,break,fix\} \\
\actionsSmallLargeModel{CS} &=& \{req\} \\
\end{eqnarray*}
\end{exmp}
%
% Let $\interfaceWithS{H}$, $H \in \lagroup{M}$, denote the set of action types which $H$ shares with one or more of $\mo{M}$'s \emph{small} groups.
%\[\interfaceWithS{H} = \{ \ \alpha\  | \ \alpha \in \interface{M}{H} \wedge (\ \coop{M}{H}{\alpha} \cap \smgroup{M} \not= \emptyset\ )\  \}\]
%Given $\actions{H}$ and $\interfaceWithS{H}$, we can calculate $\actionsLarge{H}$, $H \in \lagroup{M}$, which represents the action types in $H$\rq{}s interface, but shared with \emph{no small groups}; $\actionsLarge{H} = \actions{H} - \interfaceWithS{H}$. Note that this set includes the action types shared with other \emph{large} groups, if such action types exist. For model $\mo{M}$, the set of action types, specifically related to \emph{all} large groups, is therefore:
%\[\actionsLargeModel{M} = \bigcup_{H \in \lagroup{M}}^{} \actionsLarge{H}.\]
%Given this, the set of action types influenced by the small populations is: 
%\[\actionsSmallModel{M} = \left( \bigcup_{H \in \group{M}}^{} \actions{H} \right) - \actionsLargeModel{M}.\]
%where the first terms on the right hand side describes all the action types introduced in the model. 

\subsubsection{Identifiable Sub-Chains}
Let us assume that the model $\mo{M}$ satisfies Condition \ref{aggregationCondition}. 
In $\mo{M}$\rq{}s CTMC, let us focus on transitions of type $\actionsLargeModel{M}$.
According to the discussion above, each of these transitions changes the state of one or more large groups only, without affecting the configuration of the small ones.
Using this, the whole CTMC can be divided into sub-chains where the states within each sub-chain are connected by $\actionsLargeModel{M}$ transitions and across these, the configuration of the instances in the small groups remains the same. 
%A sub-chain is simply regarded as a sub-set of states in the CTMC. 
Formally, from a state $S$, a sub-chain $Y_i$, which can be regarded as a sub-set of states, can be derived using the following rules: 
\begin{eqnarray*}
1.&& S \in Y_i \ \wedge\ S \stackrel{(\alpha,\cdot)}{\longrightarrow} S^{\prime}\  \wedge\  \alpha \in \actionsLargeModel{M} \implies S^{\prime} \in Y_i \\
2.&& S \in Y_i \ \wedge\ S^{\prime\prime} \stackrel{(\alpha,\cdot)}{\longrightarrow} S\  \wedge\  \alpha \in \actionsLargeModel{M} \implies S^{\prime\prime} \in Y_i
\end{eqnarray*}
The sub-chain associated with a state $S$ consists of $S$, the states from which $S$ can be reached by transitions of type in $\actionsLargeModel{M}$, and the states reachable from $S$ by such transitions. These transitions capture the dynamics of the large groups in that sub-chain. 

Using the rules above, given $\mo{M}$, $\smgroup{M}$ and $\lagroup{M}$, for $\mo{M}$'s underlying CTMC, the partition $Y_{\mo{M}} = \{Y_1,Y_2,\ldots\}$ can be constructed where each $Y_i$ is a sub-chain. The state transitions inside a sub-chain are due to the changes in large groups only. Each sub-chain can be uniquely identified by the configuration it captures for the small groups, i.e. the vector $\boldsymbol{\xi}_{s}$. Two states $S_1$ and $S_2$ in the original CTMC belong to two different sub-chains if they do not record the same configuration for instances of groups in $\smgroup{M}$.

\begin{exmp}
In Fig. \ref{fig:fullstatesapce}, the CTMC of Model \ref{model1}, the sub-chains can be visually detected. Using the integer state identifiers, the following partition can be constructed for this state space: 
\[Y_{\mo{CS}} = \{\ \{1,2,3\},\{4,5,6\}\},\ldots,\{16,17,18\}\ \}\]
Note that in each sub-chain, the clients change their internal state via $think$ activities without affecting the servers. As an example, consider state $\langle S_i,S_l,S_b,C_r,C_t\rangle = \langle0,2,0,0,2\rangle$. Once the activity $(think,r_t\times2)$ takes place, the state of the $Clients$ changes. In the next $think$ transition, moving the system from state $\langle0,2,0,1,1\rangle$ to $\langle0,2,0,2,0\rangle$, again the clients change their internal state. However, across these transitions, the configuration of the servers remains the same. 
Had the model had a larger population for the clients, one would have observed very \emph{long} thread of states across each sub-chain, capturing the internal dynamics of the clients where the configuration of the servers remained unchanged. 
\end{exmp}


\subsubsection{Existence of Unlikely Boundary States and Blocked Activities}
% states in the sub-chains and the transitions. 
Before showing the next structural property, we need to define the notion of boundary states. In $\mo{M}$\rq{}s CTMC, consider an arbitrary sub-chain $Y_i$, a state $S$ within it and $\alpha \in \actions{M}$. 

As the first case, assume that $\alpha \in \actionsLargeGroup{M}$. 
Here, the small groups do not participate in $\alpha$ activities. 
Therefore, in any state $S\in Y_i$, the status of $\alpha$, i.e. whether $S$ enables $\alpha$ activities or not, depends only on the configuration of the large groups in that state. 
As the second case, assume that $\alpha\in \actionsSmallModel{M}$.
Here, the large groups do not participate in the $\alpha$ activities and therefore, in any state $S\in Y_i$, the status of $\alpha$, depends only on the configuration $S$ captures for the small groups. 
In fact, in this case, given that the configuration of the small groups is identical across all the states in $Y_i$, one can attribute the status of $\alpha$, not just to the constituent states of the sub-chain, but indeed to $Y_i$ as a whole. 

The last and more complicated case is when $\alpha \in \actionsSmallLargeModel{M}$. Here, the $\alpha$ activities are shared between small and large groups and the status of $\alpha$ in any state depends on the configurations of both small and large groups in that state. As a result of this multi-dependency, from all states in $Y_i$, we can identify a sub-set, where $\alpha$ activities are not enabled because of the large groups not enabling that action type, regardless of the configuration of the small groups. Extending this to all action types in $\actionsSmallLargeModel{M}$, in each sub-chain $Y_i$, we can find a sub-set of states where one or more action types $\alpha$ remain disabled specifically due to the lack of cooperation from the instances in the large groups. For $Y_i$, let us refer to this sub-set as $Y_i$\rq{}s collection of boundary states or $bo(Y_i)$.  
As an example, in a communication network, which consists of a small group of servers and a large group of clients, a boundary state represents a situation where some servers are ready for offering the service, but the actual service never takes place because no client requests it. Obviously, in any over-loaded system, the probability of being in boundary states is nearly zero as in these systems the resources are usually highly utilized. The formal characterisation of the boundary states follows. 
\begin{mydef}
In a model $\mo{M}$, for a state $S$ with the state vector $\boldsymbol\xi= \langle\ \boldsymbol\xi(H_1),\ldots,\boldsymbol\xi(H_{N_{\mo{M}}^{H}})\ \rangle$ in numerical vector form,
\begin{multline*}
S \ \  \text{is a boundary state} \iff \\
 \ \exists\  H_s \in \smgroup{M} \ \  \exists\  \alpha \in (\actions{H_s}\  \cap \actionsSmallLargeModel{M})\ \ \exists\  H_l \in (\lagroup{M} \cap \coop{M}{H_s}{\alpha})\ ,\\ 
\ \ \ \ \ r_{\alpha}^{*}(H_{l})=0 
\end{multline*} 
\end{mydef}

Note that for a $H_{l} \in\ \lagroup{M}$ and $\alpha \in \actionsSmallLargeModel{M}$, the sequential processes in $H_{l}$ can undertake $\alpha$ activities only passively. Here, the rules shown in Eq.	 \ref{eqn:passiveRateRules} can be used to calculate $r_{\alpha}^{*}(H_{l})$. 

For a boundary state $S_b \in bo(Y_i)$, it would be useful to find the action types which are blocked in that state. 
\begin{multline*}
bl(S_b)  =  \left\{\ \alpha \mid \exists\ H_s\  \in\ \smgroup{M} : \left[ \ \  \alpha \in (\actions{H_s}\ \cap\ \actionsSmallLargeModel{M}) \ \ \wedge \right. \right.   \\ 
\left.\left. \exists\  H_l\  \in\  (  \lagroup{M}\  \cap\  \coop{M}{H_s}{\alpha} ) : r_{\alpha}^{*}(H_l)=0 \vphantom{\actionsSmallLargeModel{M}} \ \right]  \ \ \right\} 
\end{multline*}
A related notion is $bo(Y_i,\alpha)$, representing the states in $Y_i$ where the action type $\alpha$ is blocked: 

\[bo(Y_i,\alpha) = \left\{ S \mid S \in Y_i \ \wedge\ \alpha \ \in bl(S)  \right\}.\]

\begin{exmp}
In the CTMC of Fig \ref{fig:fullstatesapce}, the set of boundary states is: 
\[\{\langle2,0,0,0,2\rangle,\langle1,1,0,0,2\rangle,\langle0,2,0,0,2\rangle,\langle1,0,1,0,2\rangle,\langle0,1,1,0,2\rangle,\langle0,0,2,0,2\rangle  \}\]
As a few examples:
\begin{eqnarray*}
bo(Y_{\langle2,0,0\rangle},req)&=&\{2,0,0,0,2\} \\
bo(Y_{\langle0,1,1\rangle},req)&=&\{0,1,1,0,2\} \\
bo(Y_{\langle0,0,2\rangle},req)&=&\{0,0,2,0,2\}
\end{eqnarray*}
\end{exmp}

\subsubsection{Rate Regularities}
Consider model $\mo{M}$, a large-scale model with small groups which satisfies \mbox{Conditions \ref{aggregationCondition}}. In its CTMC, consider a sub-chain $Y_i$ and a state $S_i \in Y_i$. 
Assume that there exists a cross-sub-chain transition $S_i \stackrel{(\alpha,R)}{\longrightarrow} S_j$ where $S_j \in Y_j$, $Y_j \not= Y_i$ (see Fig. \ref{fig:similarBehaviours}). Clearly, $\alpha\  \in \ (\actionsSmallModel{M}\ \cup\actionsSmallLargeModel{M}$).  
Having assumed that such a transition exists, then, for any state $S_i^{\prime} \in Y_{i}$ where an $\alpha$ activity is enabled, we can observe a similar transition $\transition{S_i^{\prime}}{S_j^{\prime}}{\alpha,R^{\prime}}$ where $S_j$ and $S_j^{\prime}$ are located in the same sub-chain $Y_j$ and $R=R^{\prime}$.
\begin{lemma}
\label{observation}
The above observation is formally expressed as follows: 
\begin{multline*}
\forall\  \alpha \in (\actionsSmallLargeModel{M}\ \cup\ \actionsSmallModel{M})\ ,\ \  \forall\   S_i\  \in\  Y_i\ ,\ \  \forall\  S_j\  \in\  Y_j  \\
 \left(\  \transition{S_i}{S_j}{\alpha,R} \implies 
\forall\ S_i^{\prime}\ \in\ (Y_i - bl(Y_i,\alpha)) \right. \\
 \ \ \ \left. \left[\  r_{\alpha}^{*}(S_i^{\prime}>0) \implies \exists\ S_j^{\prime}\  \in\  Y_j\ \ \ \transition{S_i^{\prime}}{S_j^{\prime}}{\alpha,R} \ \right]\  \right)
\end{multline*}
\end{lemma}

% The figure for regularities.
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth,height=0.25\textheight]{./graphs/regularities.pdf}
\caption{The non-boundary states in a sub-chain presenting similar behaviours.\label{fig:similarBehaviours}}
\end{figure}

This property expresses that for any two sub-chains $Y_i$ and $Y_j$, if, with activities of type $\alpha$, the states from $Y_i$ move into states within $Y_j$, then, the rates of these activities (transitions) are exactly the same. 
Moreover, the rule says that in any one sub-chain, all non-boundary states enable the same set of activities and with equal rates respectively. 
Based on this observation, we can define $r(\alpha,Y_i,Y_j)$, $\alpha \in \actionsSmallLargeModel{M}\ \cup \actionsSmallModel{M}$, $Y_i,Y_j\in Y_{\mo{M}}$, which denotes the rate of any $\alpha$ activity which is capable of moving a state $S_i$ in $Y_i$ to another state $S_j$ in $Y_j$, assuming that $S_i$ enables such an action type. 
\begin{eqnarray*}
r(\alpha,Y_i,Y_j) & = & \left\{
\begin{array}{ll}
r & \ \ \ \ \ \ \text{if}\ \ \ \ \ \exists\ S_i \in Y_i\  S_j \in Y_j\ , \ \ \ \transition{S_i}{S_j}{\alpha,r} \\
0 & \ \ \ \ \ \ \text{otherwise} 
\end{array} \right . 
\end{eqnarray*}

Between two sub-chains $Y_i$ and $Y_j$, there might be transitions of more than one type which connect their states (see Fig. \ref{fig:similarBehaviours}). 
Using $r(\alpha,Y_i,Y_j)$, we can define $r(Y_i,Y_j)$ to represent the total rate at which non-boundary states in $Y_i$ transition into a corresponding state in $Y_j$. 
\begin{eqnarray*}
r(Y_i,Y_j) & = & \sum_{\alpha\in(\actionsSmallModel{M}\ \cup\  \actionsSmallLargeModel{M})}^{}\ r(\alpha,Y_i,Y_j)
\end{eqnarray*}

% The figure for regularities.
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth,height=0.25\textheight]{./graphs/regularities-rates}
\caption{The rate for any one cross-sub-chain transition.}
\end{figure}

Lemma \ref{observation} holds except for the set of blocked states in $bl(Y_i,\alpha)$; for $S_b \in bl(Y_i,\alpha)$, no $\alpha$ activities are enabled. 
However, these states can be ignored as the probability of being in them is nearly zero.

\begin{exmp}
In Fig. \ref{fig:fullstatesapce}
, the activities of type in $\actionsSmallModel{CS}\ \cup\actionsSmallLargeModel{CS} = \{req,log,break,fix\}$ cause the system to leave the sub-chain it resides in and move into a new one. The rate of such activities depends on the configuration of the servers only. Across the states which reside in one sub-chain, the state of the servers does not change. Therefore, across these, the rate of any activity of type $\actionsSmallModel{CS}\ \cup\actionsSmallLargeModel{CS}$, if enabled, is the same. 

The state $2$ from the sub-chain $\{1,2,3\}$ can move into state $4$ in sub-chain $\{4,5,6\}$ via activity of type $req$ with rate $2\times r_s$. The similar transition is possible from state $3$ into state $5$ with the same rate. Moreover, states 4 and $5$ belong to the same sub-chain.
\[r(\{1,2,3\},\{4,5,6\},req) = 2\times r_s\]
Here, only activities of one action type connect some states in sub-chain $\{1,2,3\}$ to corresponding states in $\{4,5,6\}$. Therefore,
\[r(\{1,2,3\},\{4,5,6\}) = 2\times r_s\]

The states $\{2,3\}$ move respectively into the states $10,11,12$ via activities of type $brk$ with rate $2\times r_f$. Therefore $r(\{1,2,3\},\{4,5,6\},brk) = 2\times r_f$. Similar observations can be made for other sub-chains and other activities of type in $\actionsSmallModel{CS}\ \cup\actionsSmallLargeModel{CS}$. 
\end{exmp}

% possibilty of the aggregation. 
For a large-scale model $\mo{M}$ that satisfies Condition \ref{aggregationCondition}, one can construct its CTMC and using $\actionsSmallModel{M}$, $\actionsLargeModel{M}$, $\actionsSmallLargeModel{M}$, detect the sub-chains are formed and observe the rate regularities with respect to cross-sub-chain transitions. 
Moreover, it can be assumed that the probability of the model experiencing the boundary states is negligible. 
% building the aggregated CTMC.
These features exhibited by the CTMC enables us to build an aggregated CTMC for the model. 
In this CTMC, each sub-chain of the original CTMC is represented by a single aggregate state. The aggregate state associated with a sub-chain abstracts away from the dynamics of the large groups in that sub-chain and only captures the un-changed configuration the sub-chain exhibits for the small groups. 
As the result of this abstraction, the aggregated CTMC captures only the evolution of the model\rq{}s small groups and the information about the behaviour of the instances in the large groups is lost. 
The aggregate CTMC is useful because it still provides the means for studying some aspects of the system's stochastic behaviour; the evolution of the instances of the groups in $\smgroup{M}$ can be studied in a fined-grained manner without building the very large original CTMC. 

% example for the client server system
\begin{exmp}
For the client-server model, its aggregated CTMC is shown in Fig. \ref{fig:aggStateSpace}.  It shows how the state variables related to the servers behave. 
\begin{figure}
\centering
\includegraphics[width=0.48\textwidth,height=0.37\textwidth]{./graphs/ClientServerModelWithBreakdown2Servers2Clients-Aggregated}
\caption{The aggregated state space of the client-server model.\label{fig:aggStateSpace}}
\end{figure}
\end{exmp}

For this example, the aggregated CTMC was manually derived by a careful structural analysis of the model's original CTMC. In the following, we will propose an automated aggregation algorithm applicable to all large-scale PEPA models with small groups which satisfy the aggregation condition. 

%The aggregation method derives the aggregated CTMC directly from the model and avoids computationally expensive construction of the original CTMC. 



% ---------------------------------
%	An interesting piece of text that I can use somewhere in the paper. 
% ---------------------------------


%Often, in a communication system, the resources (which are of different types) smaller in number than the resource users. In our terminology, such resources constitute the small groups. As these resources significantly affect the system's performance, an important step in the performance study of the system is to derive the space of the states experienced by the resources and calculate the related probability distribution. This helps to quantitatively predict the probability of the resources being in critical conditions and the system exhibiting unsatisfactory behaviours. The aggregation introduced above facilitates construction of an aggregated CTMC which only focuses on the dynamics of the system's small groups without capturing the evolution of the large ones. 




% ---------------------------------
%	some examples.
% ---------------------------------

%For example, in the CTMC of Fig. \ref{fig:fullstatesapce}, consider the state $\langle2,0,0,1,1\rangle$ where there are two idle servers, a client who is requesting and another one who is thinking. 
%A $req$ transition moves this state into $\langle1,1,0,0,2\rangle$ with rate $2\times r_s$ (there are two instances of an idle servers in the enabling state). 
%Although $req$ is a shared activity, its  rate does not depend on the state variables associated with the clients. 


%property
%A consequence of the second property is that, across the states that reside in one sub-chain, the rate of any transition whose type is in \mbox{$\actionsSmallModel{M}$}, does not change. 
%example
%For example, consider the sub-chain 
%\[\langle0,2,0,0,2\rangle \longrightarrow\langle0,2,0,1,1\rangle \longrightarrow  \langle0,2,0,0,2\rangle.\] 
%As the state of the servers do not change, the rates of the transitions enabled by the servers ($req$, $log$, $break$, $fix$) remain the same. Additionally, firing of one of these transitions moves the system from the above sub-chain into another sub-chain which exhibits a similar structure in terms of the dynamics of the clients. For example, the instances of $(log,r_l)$ move the system from the above sub-chain to the states of the following sub-chain which presents a similar structure.
%\[\langle1,1,0,0,2\rangle \longrightarrow \langle1,1,0,1,1\rangle \longrightarrow \langle1,1,0,2,0\rangle.  \]
%Note that the state of the servers is different in the new sub-chain.

%-----------------------------
% Some text about the rates. 
%-----------------------------

%The transition of a type $\alpha$ which moves the states of one sub-chain to the states of another, changes the state variables related to some small groups. Moreover, if $\alpha$ is shared and some of the large groups enable $\alpha$; i.e. $\alpha \in En^{*}(H)\ ,\ H \in \lagroup{M}$, then the state of the relative large groups will also change. As the state of the small groups does not change in one sub-chain, each sub-chain can be identified by the state it holds for the small groups; .




==> Algorithm/algorithm.tex <==
\section{Aggregation Algorithm}
\label{aggregationAlgorithSection}
The aggregated CTMC of a conforming model $\mo{M}$ is more abstract than its original CTMC in the sense that the former only captures the dynamics (the state and the transitions) of the instances in $\smgroup{M}$ whilst the latter captures the dynamics of instances in all groups. Specifically, the aggregate CTMC's structure is independent of the sizes defined for the model's large groups; if, for some groups, their size change, as long as $\lagroup{M}$ is not altered, then the model will have exactly the same aggregated CTMC. 
This independence justifies the development of an algorithm which directly builds the aggregated CTMC from the model (see Fig \ref{fig:ways}). 
This algorithm, in its first step, called the reduction step, transforms the system equation of the original model $\mo{M}$ into a \emph{reduced} system equation which captures $\mo{M}$'s structure only with respect to the group in $\smgroup{M}$. Let us call this $\mo{M}_{R}$. 
In the next step, using $\mo{M}_{R}$ and a semantics developed for PEPA population models, the aggregated CTMC is generated. We will cover these steps in this section. 
% The reduction takes care of book-keeping about the synchronizations. 
Note that the reduced system equation is faithful in terms of capturing the synchronization restrictions imposed on any of the small groups. Although the large groups are removed from the model, the reduction rules guarantee that the behaviour exhibited considering $\mo{M}_{R}$ matches the one seen for $\smgroup{M}$ in the original CTMC;
\[\forall \ H \in \smgroup{M}\ ,\ \ \coop{\mo{M}_R}{H}{\alpha} = \coop{M}{H}{\alpha}\  \cap\   \smgroup{M} \]
%We will cover this property in more detail in Section X.

\begin{figure}[]
\centering
\includegraphics[width=0.9\textwidth,height=0.35\textheight]{./graphs/Algorithm}
\caption{Ways to the aggregated CTMC.\label{fig:ways}}
\end{figure}

\subsection{Reduction}
The rules below will be applied to the input model $\mo{M}$'s system equation in order to produce the reduced model $\mo{M}_R$. 
\begin{eqnarray*}
red({G}) & = & \left\{\begin{array}{ll}
											red({G}_1) \mysync{L} red({G}_2) & \text{if}\ \ {G} = {G}_1  \mysync{L}  {G}_2  \\ \\
											H\{\cdot\} & \text{if}\ \ {G}=H\{\cdot\} \ \wedge \  H \in \smgroup{M}	\\ \\
											Nil & \text{if}\ \ {G}=H\{\cdot\} \ \wedge \  H \in \lagroup{M}	\\ \\ 
											red(X) & \text{if}\ \ {G} \rmdef X \\
										\end{array} \right.   \\ 
\end{eqnarray*}
The process $Nil$ represents a sequential process which does not undertake any activity. Applying the rules results in a system equation where all large groups are replaced by this process. The following rules removes $Nil$ processes to find the reduced system equation in its final shape:
\begin{eqnarray*}
1.&& Nil \mysync{\cdot} Nil = Nil\\
2.&& Nil \mysync{\cdot} P = P
\end{eqnarray*}
\begin{exmp} Consider Model \ref{model2}, an extension of the previous client-server model.
\begin{model}
\begin{eqnarray*}
C_{think} & \rmdef & (think, r_{t}).C_{req}\  \\
C_{req} & \rmdef & (req, {\top}).C_{thinking} +\ (ask,\top).C_{think} \\ \\
S_{idle} & \rmdef & (req, {r_{s}}).S_{log} \\
S_{log}  & \rmdef & (log, r_l).S_{idle} \   \\ \\
S_{ready} & \rmdef & (ask,{r_a}).S_{proc} \\
S_{proc} & \rmdef & (process,r_p).S_{ready} \\\\
 \mathbb{CS}^{\prime} & \rmdef & \left( \  Servers\{\ S_{idle}[n_s]\  || \  {S_{log}[n_l]}\ \} \mysync{\{ req\}} \right. \\ 
 && \left . Clients \{\ C_{think}[n_c]\  ||\   {C_{req}[n_r]}\ \}\ \vphantom{\mysync{\{ ask\}}} \right )  \mysync{\{ ask\}}   Servers^{\prime}\{\ S_{ready}[n_r]\  || \  {S_{proc}[n_p]}\ \}
\end{eqnarray*}	
\caption{A client-server model where there are servers of two types interacting with the clients.\label{model2}}
\end{model}
In this, there are servers of two different types synchronising with the clients. When a client instance has finished with thinking, it can either undertake a shared activity $req$ with an instance of a server in group $Servers$ or it can undertake the activity $ask$ with a server instance in group $Server^{\prime}$. The behaviour of the instances in $Servers$ is like before. A server which performs an ask, moves into state $S_{proc}$ in which it processes the question just received. Upon finishing its processing, it moves into the $S_{ready}$ state again. 

In this model, the population of the clients is assumed to be large. Therefore, $\lagroup{CS^{\prime}} = \{Clients\}$ and $\smgroup{CS^{\prime}}=\{Servers, Servers^{\prime}\}$. Using the rules above, the reduced version of the system equation is: 
\begin{eqnarray*}
\mathbb{CS}^{\prime}_R = red(\mathbb{CS}^\prime) & = &  (\ S_{idle}[n_s]\  || \  {S_{logging}[n_l]}\ )  \mysync{\{ request,ask\}} (S_{ready}[n_r]\  || \  {S_{processing}[n_p]})
\end{eqnarray*}
where the $Clients$ group is removed from the equation.
\end{exmp}
\subsection{Semantics}
\label{semanticsSection}

Having built the reduced form of the system equation, we apply the \emph{count-oriented structured operational semantics} to derive the model\rq{}s underlying labelled transition system in numerical vector form. 

% previous grouped PEPA semantics.
Based on Hillston\rq{}s semantics for PEPA \cite{Hillston:1996}, Hayden and Bradley, in \cite{Hayden:2010}, proposed a set of semantic rules for generating the underlying labelled transition systems (LTS\footnote{In general terms, a labelled transition system consists of a set of states, a set of transition labels and a transition relation.
This system is used to generate the grouped PEPA model\rq{} underlying CTMC.}) of grouped PEPA models. 
In these transition systems, the states are process algebra terms in which the state of each sequential process involved in the model is separately captured; the semantics does not directly give rise to a transition system based on the counting abstraction.
In this system, the evolution of each instance is captured regardless of the fact that the model contains large numbers of them. 
As a simple example, if a sequential process $P$ enables an $\alpha$ activity ($P \stackrel{(\alpha,r)}{\longrightarrow}  P^{\prime}$) and the system consists of an array of $n$ copies of $P$ ($S \rmdef P[n]$), then, using Hayden and Bradley\rq{}s semantics, in the model\rq{}s LTS, the transition 
$P[n] \stackrel{(\alpha,r)}{\longrightarrow} P^{\prime}\ |\  P[n-1]$, where the first $P$ in the array is engaged, is recorded separately from the similar transition 
$P[n] \stackrel{(\alpha,r)}{\longrightarrow} P\ |\  P^{\prime}\  |\  P[n-2]$, where the second instance is engaged and so on. According to the counting abstraction, in such cases, $P$ instances should not be treated separately and for their population\rq{}s one step $\alpha$ evolution, one transition
$P[n] \stackrel{(\alpha,r \times n)}{\longrightarrow} P^{\prime}[1]\ |\  P[n-1]$ is recorded (with a modified rate) in the state space. 
The applicability of the Hayden and Bradley\rq{}s semantics for the state space generation of large-scale models is hindered as it does not employ a compact state representation method. 

% count-oriented semantics
% in line with Stephen\rq{}s aggregation algorithm. 
The count-oriented semantics is similar to the \emph{equivalence-aware} semantics offered by Gilmore et al. in \cite{922715}. 
There, the idea of canonical states is adopted when building a model\rq{}s underlying  LTS.  
Two states are canonically equal if they satisfy the \emph{strong equivalence} condition defined for stochastic processes\footnote{For the formal definition of strong equivalence, please read \cite{Hillston:1996}, Def. (7.2.1)}.
This equivalence condition allows us to determine if two states are equal, at the population level, even when at the level of individual sequential processes, they are different. 
The states which are canonically equivalent, will be represented by a single canonical state when building the state space.
(eg. both processes $P\ |\ P^{\prime}[1]\ |\ P[n-2]$ and $P[n-1]\ |\ P^{\prime}[1]$ are canonically equal as both capture the same configuration at the population level). Using the canonical states, Gilmore\rq{}s et al. semantics is essentially following the counting abstraction and therefore, the generated LTS is more abstract and compact than that constructed by Hayden and Bradley semantics. 

Two features distinguish the count-oriented semantics from the equivalence-aware semantics. First, the count-oriented semantics is specifically designed for grouped PEPA models where as the equivalence-aware one supports normal PEPA models.
Second, in the state space generated by the latter, the process algebra terms are still present in each state and if, one is interested in state representation based on numerical counters, then an additional translation step would be required. However, the count-oriented semantics operates at the level of state counter and it directly results in a state space in numerical vector form. Regardless of these minor distinctions, the two semantics follow the same operational steps.
 	
\begin{framed}

\begin{itemize} 
\item Constant: 
\begin{eqnarray*}
&&\inference []
{M \stackrel{(\alpha,r)}{\longsquiggly} M^{\prime}} 
{A \stackrel{(\alpha,r)}{\longsquiggly} M^{\prime}}\ A \rmdef M
\end{eqnarray*}
\item Promotion of a sequential component's transition to the group level:
\begin{eqnarray*}
&&\inference []{C_{x,y} \stackrel{(\alpha,r_{\alpha})}{\longrightarrow} C_{x,y^{\prime} }}
{\boldsymbol\xi(H) \stackrel{(\alpha,\xi(H,C_{x,y})r_{\alpha}(C_{x,y},C_{x,y^{\prime}}))}{\verylongsquiggly}\Theta(\boldsymbol\xi(H),C_{x,y},C_{x,y^{\prime}})} \ \xi(H,C_{x,y})>0
\end{eqnarray*}
\item Cooperation between groups:
\begin{eqnarray*}
& \inference[]{\boldsymbol\xi(H_i) \stackrel{(\alpha,r(\boldsymbol\xi(H_i)))}{\longsquiggly} \boldsymbol\xi^{\prime}(H_i) }
{\boldsymbol\xi(H_i) \mysync{L} \boldsymbol\xi(H_j)\stackrel{\alpha,r(\boldsymbol\xi(H_i)))}{\longsquiggly} \boldsymbol\xi^{\prime}(H_i)\mysync{L}\boldsymbol\xi(H_j)}&\alpha \not \in L 
\\
& \inference[]{\boldsymbol\xi(H_j) \stackrel{(\alpha,r(\boldsymbol\xi(H_j)))}{\longsquiggly} \boldsymbol\xi^{\prime}(H_j) }
{\boldsymbol\xi(H_i) \mysync{L} \boldsymbol\xi(H_j)\stackrel{\alpha,r(\boldsymbol\xi(H_j)))}{\longsquiggly} \boldsymbol\xi(H_i)\mysync{L}\boldsymbol\xi^{\prime}(H_j)}&\alpha \not \in L 
\\
&\inference[]{\boldsymbol\xi(H_i) \stackrel{(\alpha,r_1(\boldsymbol\xi(H_i)))}
{\longsquiggly} \boldsymbol\xi^{\prime}(H_i) \ \wedge \ \boldsymbol\xi(H_j) \stackrel{(\alpha,r_2(\boldsymbol\xi(H_j)))}{\longsquiggly} \boldsymbol\xi^{\prime}(H_j)}{\boldsymbol\xi(H_i) \mysync{L} \boldsymbol\xi(H_j)\stackrel{(\alpha,R)}{\longsquiggly} \boldsymbol\xi^{\prime}(H_i)\mysync{L}\boldsymbol\xi^{\prime}(H_j)} & \alpha \in L \\
& R = \frac{r_1(\boldsymbol\xi(H_i))}{r^{*}_{\alpha}(H_i)} \frac{r_2(\boldsymbol\xi(H_j))}{r^{*}_{\alpha}(H_j)} min(r^{*}_{\alpha}(H_i),r^{*}_{\alpha}(H_j)) & 
\end{eqnarray*}
\end{itemize}
\end{framed}

% this semantics is not sufficient for building the transition relation. 
% construction of the count-oriented transition relation is depends on construction of the transition relation by PEPA original semantics for the sequential components. 

The rules for constructing the transition relation $\shortsquiggly$ make use of the LTS constructed by the original semantics rules in \cite{Hillston:1996}. However, note that this LTS, which embeds in it the transition relation $\rightarrow$ (see the premise of the first rule), needs to be constructed only at the level of the model\rq{}s sequential processes; for each sequential process in the model an automata is constructed which captures the states and transitions that each instance of the sequential process experiences (in this LTS, the transition relation $\rightarrow$ captures how the local states of the sequential processes are connected). The model\rq{}s system equation and the information captured by this LTS is enough to derive the model\rq{}s behaviour in terms of numerical vectors associated with the model\rq{}s groups (see Section \ref{preliminaries}). 

If a sequential process in state $C_{x,y} \in ds^{*}(H)$ is capable of undertaking $\alpha$ and becoming $C_{x,y^{\prime}}$, then when \mbox{$\xi(H,C_{x,y}) > 0$}, the transition can be fired by any such $C_{x,y}$ instance in $H$. This will change the state (some of the counters) associated with $H$. The function $\Theta(\boldsymbol{\xi}(H),C_{x,y},C_{x,y^{\prime}})$ outputs the updated version of $\boldsymbol{\xi}(H)$ when an instance in $H$ with state $C_{x,y}$ becomes $C_{x,y^{\prime}}$; in $\boldsymbol{\xi}(H)$ it decreases $\xi(H,C_{x,y})$ by one and increases $\xi(H,C_{x,y^{\prime}})$ by one. 

The cooperation rules show how the state vector of the cooperating groups change simultaneously. Note that one rule is omited. 

% definition of function theta
\begin{eqnarray*}
\Theta(\boldsymbol{\xi}(H),C_{x,y},C_{x,y^{\prime}}) & = & \langle\  \Theta^{\prime}(\boldsymbol{\xi}(H),C_{x,y},C_{x,y^{\prime}},\xi(H,C^{\prime\prime})) \mid c^{\prime\prime}\in ds^{*}(H)\ \rangle \\
\Theta^{\prime}(\boldsymbol{\xi}(H),C_{x,y},C_{x,y^{\prime}},\xi(H,C^{\prime\prime}) & = & \left\{
\begin{array}{ll}
\xi(H,C^{\prime\prime})-1 &  \ \ \ \ \ \text{if}\ \ \ C^{\prime\prime} = C_{x,y}\\
\xi(H,C^{\prime\prime})+1 &  \ \ \ \ \ \text{if}\ \ \ C^{\prime\prime} = C_{x,y^{\prime}}\\
\xi(H,C^{\prime\prime})	 &  \ \ \ \ \ \text{otherwise}\ \ \ 
\end{array}\right.
\end{eqnarray*}

\subsection{Generating the Aggregate CTMC}

In the context of our aggregation algorithm, the count-oriented semantics will be applied on the reduced form of a model\rq{}s system equation to form its aggregated LTS. For a model $\mo{M}$, this LTS, which is formally characterised below, captures how the instances of groups in $\smgroup{M}$ evolve and constitutes the model\rq{}s aggregated CTMC.

\textbf{Derivative Set}. The derivative set of a state $S$, denoted by $D^{*}(S)$, is the smallest set of states satisfying the following conditions. Intuitively, $D^{*}(S)$, finds all the states reachable from $S$ using $\shortsquiggly$. 
\begin{itemize}
\item $S \in D^{*}(S)$.
\item If $S_1 \in D^{*}(S)$ and $S_1 \stackrel{(\alpha,\cdot)}{\shortsquiggly} S_2 $ then $S_2 \in D^{*}(S)$.
\end{itemize}

\textbf{Aggregated Labelled Transition System} is defined as a tuple \mbox{$(D^{*}(S_0),\Omega,\shortsquiggly)$}. $S_0$ is the model's initial aggregate state; i.e the state vector capturing the state $\mo{M}_R$ shows. $\Omega = (\mathcal{A} \times \mathcal{F} ) $ is the transition system's alphabet where $\mathcal{A}$ is the set of action types defined in the model and $\mathcal{F}$ is a function space defined over $\mathbb{Z}_{+}^{d_{\mo{M}_R}}$. Here, $d_{\mo{M}_R}$ is the dimension of the reduced system equation. Each member function of $\mathcal{F}$ corresponds to an action type; the member $F_{\alpha}$ defines the rate of observing an activity of type $\alpha$ in the vector space $\mathbb{Z}_{+}^{d_{\mo{M}_R}}$. 

\begin{exmp} Consider Model \ref{model2}. The CTMC in Fig. \ref{fig:aggStateSpace} shows the model's aggregate CTMC when $n_s=n_r=1$ and $n_l=n_p=0$. The population of the clients does not affect the structure of this aggregate CTMC.
\end{exmp}


==> CalculatingMarginals/calculatingMarginals.tex <==
\section{Calculating Marginal Probability Distributions}
\label{calculatingMarginalDistributionSection}
\subsection{Aggregated CTMC as the Source of Marginal Distributions}
\label{equationAlgorithm}
The underlying numerical state vector $\boldsymbol{\xi}$ of a PEPA model can be regarded as a vector of dependent random variables.
% where each variable (counter) $\xi(H,C_{x,y})$ counts how many instances are currently representing the behaviour associated with one local state $C_{x,y}$. 
The model\rq{}s CTMC shows how these random variables evolve.
Using this CTMC, a system of linear differential equations, also knows as Chapman-Kolmogorov equations (hereafter, the C-K equations), can be derived and the solution of these equations shows the \emph{joint} probability distribution of the state random variables at any given time.
For a model, the number of equations in its C-K system is equal to the number of states the model\rq{}s CTMC has.
Therefore, for large-scale PEPA models, calculating their full joint probability distributions is not usually feasible. 

The state vector $\boldsymbol\xi$ of a large-scale PEPA model $\mo{M}$ which satisfies the aggregation conditions can be partitioned into two sub-vectors; $\boldsymbol\xi = \langle \boldsymbol\xi_{s}, \boldsymbol\xi_{l}\rangle$ where $\boldsymbol\xi_{s}$ captures the state of instances within groups in $\smgroup{M}$ and $\boldsymbol\xi_l$ captures the state of the instances within groups in $\lagroup{M}$. 
The aggregation algorithm proposed for these models constructs an aggregated CTMC in which the evolution of the state variables only in $\boldsymbol\xi_{s}$ is captured. 
Consequently, the aggregate CTMC can be used as the basis for calculating some \emph{marginal} probability distributions over the random variables $\xi(H,C_{x,y})\ ,\  \forall\  H_i \in \smgroup{M}\ ,\  \forall\  C_{x,y} \in ds^{*}(H_i) $. The calculation is through constructing a system of linear differential equations whose solution provides the marginal distributions. In the following, assume that $X_a$ denotes the stochastic process with behaviour captured by the aggregated CTMC. For each state in this CTMC, one equation is constructed: 
\begin{multline*}
\forall S \in ds^{*}(S_0):\  \frac{d\ \mathbb{P}(X_a = S)}{d\ t} = +\sum_{\alpha:\  S_j \stackrel{(\alpha,r_{\alpha}^{*}(\boldsymbol\xi))}{\longsquiggly} S} r^{*}_{\alpha}(\boldsymbol\xi) \times \mathbb{P}(X_a=S_j) \\ 
 - \left[\sum_{\alpha:\ S \stackrel{(\alpha,r_{\alpha}^{*}(S))}{\longsquiggly} S_j} r_{\alpha}^{*}(S)\right] \times \mathbb{P}(X_a=S)
\end{multline*}

The algorithm in Fig \ref{alg:generatingODEs} constructs this system of ODEs. In the algorithm, the following notation has been used. Let $S_i$ be a state in the aggregate CTMC. 
For $S_i$, let $in(S_i)$ denote the set of states $S_h$ from which there is a transition into $S_i$. 
Similarly, let $out(S_i)$ be the set of states into which there is a transition from $S_i$; 
\begin{eqnarray*}
in (S_i) &=& \{ S_h \mid S_h \stackrel{(\alpha,\cdot)}{\shortsquiggly S_i} \} \\
out (S_i) &=& \{ S_k \mid S_i \stackrel{(\alpha,\cdot)}{\shortsquiggly S_k} \}
\end{eqnarray*}


\mathligsoff

\begin{program}[h]
\begin{alltt}
for each aggregate state \(S\) in \(ds\sp{*}(S\sb{0})\) form one equation \(\frac{d \mathbb{P}(X\sb{a}=S)}{dt}\) as \(E\) 

\(in\sb{S} \leftarrow in(S) \)                         // calculate the set \(in(S)\)
\(out\sb{S} \leftarrow out(S) \)                       // calculate the set \(out(S)\)

    for each state \(S\sb{h} \in in(s) : S\sb{h} \stackrel{(\alpha,r\sb{\alpha}\sp{*}(\boldsymbol\xi))}{\longsquiggly} S \) 

        add  \( +\ r\sb{\alpha}\sp{*}(\boldsymbol\xi)\times\mathbb{P}(X\sb{a}=S\sb{h}) \) to \(E\)    // probability in-flux into
                                      // aggregate state \(S\)


    for each state \(S\sb{j} \in out(S) : S \stackrel{(\alpha,r\sp{*}\sb{\alpha}(\boldsymbol\xi))}{\longsquiggly} S\sb{j} \) 

        add  \(  -\ r\sp{*}\sb{\alpha}(\boldsymbol{\xi})\times\mathbb{P}(X\sb{a}=S)\) to \(E\)     // probability out-flux out of 
                                      // aggregate state \(S\)
\end{alltt}
\caption{Pseudo-code for generating the aggregated system of ODEs.\label{alg:generatingODEs}}
\end{program} 
\mathligson

\subsection{Original C-K Equations as the Source of Marginal Distributions}

%	1- for each state, the chapman-kolmogorov equation
%	2- similarity between the states which reside in a single sub-chain in terms of probability 
%	influx-outflux
% 	3- the notion of boundary states inside each sub-chain
%			these are the states where the large populations are blocking the small ones. 
%			the probability of being in them is really small. 
%	4- the description of the properties for the probability fluxes
%	5- distinction from lumpability.  % not incluced yet.
%	6- building the ODEs at the level of the sub-chains % done. 

For the complete CTMC of a PEPA model, the associated system of C-K equations captures how for each state $S$, the probability of being in $S$ changes through the probability fluxes into $S$ (from the states where there is a transition into $S$) and the probability fluxes out of $S$ (through the transitions enabled by $S$). 
For a model, constructing its system of C-K equations means that the focus of the analysis is at the level of individual states present in the model\rq{}s CTMC and the goal is to find the joint probability distribution on all state variables. 
Solving the equations gives rise to detailed information about the behaviour of the model; at any given time the probability of being in any given configuration will be known. 

% an alternative view on the analysis. 
The state space of a large-scale model which satisfies the aggregation conditions can be regarded as a collection of sub-chains, as opposed to a set of states. 
Consequently, when running the analysis, instead of being interested in the probability of the model being in particular states, one can take the alternative goal of finding the probabilities at the level of constituent sub-chains. 

In Section \ref{X}, we observed that the CTMC of a model conforming to Condition \ref{aggregationCondition}, exhibits important structural properties. In particular, Lemma \ref{lemma1}, focused on regularities with respect to the rates of the cross-sub-chain transitions.
In this section, we will see that these rate regularities give rise to similar regularities with respect to the probability fluxes coming into and going out of the sub-chains. 
This enables us to derive an approximate closed system of ODEs, from the original C-K equations, which abstracts away from the individual states and captures how the probability evolutions take place at the level of sub-chains.  
%We show that these equations co-inside with the equations which can be directly derived from the 

\subsubsection{Conversion of the Original C-K Equations}

% the probability flux for a single state.
Informally, the probability flux which is observed to flow out of a state $S$ through an activity of type $\alpha$ is a function of two factors; first, the probability of the system being in $S$ and the second, the rate at which $\alpha$ is to be fired assuming that the system is in $S$. 

% the probability flux for a sub-chain.
The probability flux out of a sub-chain $Y_i$ to another one $Y_j$ is the result of all probability fluxes moving from constituent states in $Y_i$ to corresponding states in $Y_j$ by transitions like $\transition{S_i}{S_j}{\alpha,\langle r_{\alpha,Y_i,Y_j}\rangle}$, $S_i\in Y_i$, $S_j \in Y_j$, and $\alpha \in \actionsSmallLargeModel{M}\ \cup \actionsSmallModel{M}$.  Lemma \ref{lemma} expresses that in any one sub-chain, the non-boundary states within, offer the same rate for such $\alpha$ transitions respectively. This lemma, leads us to the conclusion that in the CTMC of model $\mo{M}$ which satisfies Condition \ref{}, all probability fluxes, associated with the transitions that both have the same action type and connect the same sub-chains, share their second factor; i.e. the rate of these transitions are the same. 

% the actual conversion.
Here we show how this enables us to convert $\mo{M}$\rq{}s C-K equations into a new system of ODEs. Let $X$ be the random process with the behaviour captured by $\mo{M}$\rq{}s original CTMC. In the following  $\mathbb{P}_{\langle X=S_i\rangle}(t)$ denotes the probability that at time $t$, the random process $X$ is in state $S_i$. 
\begin{multline}
\label{simpleCKEquation}
\frac{\proba{X = S_i}}{d\ t}  =  - \sum_{\longtransition{S_i}{S_j}{\alpha,r_{\langle\alpha,S_i,S_j\rangle}}\ ,\ S_j \in Y_\mo{M}}^{} \mkern-18mu\mkern-18mu\mkern-18mu \proba{X=S_i} \times  r_{\langle\alpha,S_i,S_j\rangle}\ \ \ 
+\\
 \sum_{\longtransition{S_j}{S_i}{\alpha,r_{\langle\alpha,S_j,S_i\rangle}}\ ,\ S_j \in Y_{\mo{M}}}^{}
\mkern-18mu\mkern-18mu\mkern-18mu\proba{X=S_j} \times  r_{\langle\alpha,S_j,S_i\rangle}
\end{multline}
The probability of being in a sub-chain $Y_i$ at time $t$ is equal to the sum of the probabilities of being in any of the states in $Y_i$. 
\begin{eqnarray}
\proba{X \subset Y_i} &=& \sum_{S_i \in Y_i}^{}\ \proba{X=S_i}
\end{eqnarray}
Being interested in the probability evolutions at the level of sub-chains, for each sub-chain $Y_i$, we form one equation. $\proba{X\subset Y_i}$ denotes the probability that at time $t$, the system is in any of the states in sub-chain $Y_i$.
\begin{eqnarray}
\label{complexCKEquation}
\frac{d\  \proba{X\subset Y_i}}{d\ t} & = & \frac{d\ \sum_{S_i \in Y_i}^{}\ \proba{X=S_i} }{d\ t} = \sum_{S_i \in Y_i}^{}\ \frac{d\ \proba{X=S_i}}{d\ t}
\end{eqnarray}
In the context of a sub-chain, the probability fluxes which correspond to action types in $\actionsLargeModel{M}$ cancel each other and have no effect on the probability fluxes in and out of the whole sub-chain. 
Substituting (\ref{simpleCKEquation}) in (\ref{complexCKEquation}), we get: 
\begin{multline}
\label{eqn:bothComponents}
\sum_{S_i \in Y_i}^{}\ \frac{d\ \proba{X=S_i}}{d\ t}  =   
\sum_{S_i\ \in\ Y_i}^{} \left( 
- \sum_{\sumArray{\longtransition{S_i}{S_j}{\alpha,r_{\langle\alpha,S_i,S_j\rangle}}\ ,\ S_j\in Y_j\ }{\alpha \in (\actionsSmallLargeModel{M}\  \cup \actionsSmallModel{M})}}^{}
\mkern-18mu\mkern-18mu\mkern-18mu
 \proba{X=S_i} \times  r_{\langle\alpha,S_i,S_j\rangle} \right. \\
\left. + \sum_{\sumArray{\longtransition{S_k}{S_i}{\alpha,r_{\langle\alpha,S_k,S_i\rangle}}\ ,\ S_k \in Y_k\ }{\alpha\ \in (\actionsSmallLargeModel{M}\ \cup \actionsSmallModel{M})}} 
\mkern-18mu\mkern-18mu\mkern-18mu\proba{X=S_k} \times  r_{\langle\alpha,S_k,S_i\rangle} \right)
\end{multline} 

Considering the first term of (\ref{eqn:bothComponents}) and Lemma (\ref{observation}): 
\begin{eqnarray}
\label{eqn:firstComponent}
&& \sum_{S_i \in Y_i}{} \left(
\sum_{\sumArray{\longtransition{S_i}{S_j}{\alpha,r_{\langle\alpha,S_i,S_j\rangle}}\ ,\ S_j \in Y_j\ }{\alpha \in (\actionsSmallLargeModel{M}\  \cup \actionsSmallModel{M})}}^{}
\mkern-18mu\mkern-18mu\mkern-18mu
 \proba{X=S_i} \times  r_{\langle\alpha,S_i,S_j\rangle}\ 
\right) \\ 
\nonumber 
&= &\sum_{S_i\in Y_i}^{} \ \left(
\sum_{\sumArray{\longtransition{S_i}{S_j}{\alpha,r_{\langle\alpha,S_i,S_j\rangle}}\ ,\   S_j \in Y_j\ }{\alpha \in (\actionsSmallLargeModel{M}\  \cup \actionsSmallModel{M})}}^{}
\mkern-18mu\mkern-18mu\mkern-18mu
 \proba{X=S_i} \times r_{\langle\alpha,Y_i,Y_j\rangle}\ 
\right) \\
\nonumber & = &  \sum_{S_i\in Y_i}^{} \proba{X=S_i}\ \left(
\sum_{\sumArray{\longtransition{S_i}{S_j}{\alpha,r_{\langle\alpha,S_i,S_j\rangle}}\ ,\   S_j \in Y_j\ }{\alpha \in (\actionsSmallLargeModel{M}\  \cup \actionsSmallModel{M})}}^{}
\mkern-18mu\mkern-18mu\mkern-18mu
  r_{\langle\alpha,Y_i,Y_j\rangle}\ 
\right) \\
\nonumber & \approx &\sum_{S_i \in Y_i}^{} \proba{X=S_i} \left(
\sum_{{Y_j \in \mathbb{D}}}^{}\   r_{\langle Y_i,Y_j\rangle}\ 
\right)  \\
\nonumber & = & \left(
\sum_{{Y_j \in Y_{\mo{M}}}}^{}\   r_{\langle Y_i,Y_j\rangle}\ 
\right) \sum_{S_i \in Y_i}^{} \proba{X=S_i} \\
\nonumber & = & \left(
\sum_{{Y_j \in Y_{\mo{M}}}}^{}\   r_{\langle Y_i,Y_j\rangle}\ 
\right) \proba{X \subset Y_i}.
\end{eqnarray} 
The approximation step is based on the assumption that the probability of being in boundary states in nearly zero and therefore, the same probability fluxes as of the non-boundary ones can be associated to them. 

Similarly, for the second term of Eq. (\ref{eqn:bothComponents})
\begin{eqnarray}
\label{eqn:secondComponent}
&&\sum_{S_i \in Y_i}{} \left(
\sum_{\sumArray{\longtransition{S_k}{S_i}{\alpha,r_{\langle\alpha,S_k,S_i\rangle}}\ ,\ S_k \in Y_k\ }{\alpha \in (\actionsSmallLargeModel{M}\  \cup \actionsSmallModel{M})}}^{}\ \proba{X=S_k} \times  r_{\langle\alpha,S_k,S_i\rangle}\ 
\right)    \\
\nonumber & = & \sum_{S_i \in Y_i}\   \left(
\sum_{\sumArray{\longtransition{S_k}{S_i}{\alpha,r_{\langle\alpha,Y_k,Y_i\rangle}}\ ,\ S_k\in Y_k\ }{\alpha \in (\actionsSmallLargeModel{M}\  \cup \actionsSmallModel{M})}}^{}\ \proba{X=S_k} \times  r_{\langle\alpha,S_k,S_i\rangle}\ 
\right)  \\
\nonumber& \approx & \sum_{S_i \in Y_i}^{}\ \left(
\sum_{\transition{S_k}{S_i}{.,.}\ ,\ S_k\in Y_k}^{}\ \proba{X=S_k} \times  r_{\langle Y_k,Y_i\rangle}\ 
\right) \ \ \ \ 
\begin{array}{c}
\text{(By the negligible probability of} \\
\text{being in boundary states)}
\end{array}
\\
\nonumber& = &
\sum_{S_i \in Y_i}\ \sum_{Y_k \in Y_{\mo{M}}}\ \sum_{\transition{S_k}{S_i}{\cdot,\cdot}\ ,\ S_k \in Y_k}
\left(
\ \proba{X=S_k} \times  r_{\langle Y_k,Y_i\rangle}\ 
\right) 
\\
\nonumber& = &\sum_{Y_k \in Y_{\mo{M}}}\ \sum_{\transition{S_k}{S_i}{\cdot,\cdot}\ ,\ S_k \in Y_k}
\left(
\ \proba{X=S_k} \times  r_{\langle Y_k,Y_i\rangle}\ 
\right)  \\
\nonumber & \approx &\sum_{Y_k \in Y_{\mo{M}}}\ r_{\langle Y_k,Y_i\rangle} \times \sum_{S_k \in Y_k}\ \proba{X = S_k}  \\ 
\nonumber & = &\sum_{Y_k \in Y_{\mo{M}}}\ r_{\langle Y_k,Y_i\rangle} \times \proba{X \subset Y_k}
\end{eqnarray}
Substituting Eq. \ref{eqn:firstComponent} and \ref{eqn:secondComponent} in Eq. \ref{eqn:bothComponents}, we derive: 
\begin{eqnarray}
\label{finalEquation}
\forall\  Y_i \in Y_{\mo{M}}, \ \ \frac{d\ \proba{X \subset Y_i}}{d\ t} =  - \sum_{Y_j \in Y_{\mo{M}}}\ \proba{X\subset Y_i} \times r(Y_i,Y_j) + 
  \sum_{Y_k \in Y_{\mo{M}}} \proba{X\subset Y_k} \times r(Y_k,Y_i)
\end{eqnarray}
Eq (\ref{finalEquation}) captures the probability evolutions at the level of sub-chains.








\newpage

\begin{exmp}
Consider the client-server system of Model 1 and its complete state space in Fig. \ref{fig:fullstatesapce}. The states are annotated with integer identifiers and these numbers are used when expressing probabilities. For example, $\proba{X=\langle2,0,0,2,0\rangle} = \proba{X=1}$.
\begin{eqnarray*}
\proba{X\subset\{1,2,3\}} &=& \proba{X=1} + \proba{X=2} + \proba{X=3} \\
\frac{d\ \proba{X\subset\{1,2,3\}}}{d\ t} &=& \frac{d\ \proba{X=1}}{d\ t} + \frac{d\ \proba{X=2}}{d\ t} + \frac{d\ \proba{X=3}}{d\ t} = \\
\frac{d\ \proba{X=1}}{d\ t} & = & \proba{X=4} \times r_l - \proba{X=1}\times  r_b + \proba{X=10} \times r_f - \proba{X=1}\times 2 \times r_t \\ 
\frac{d\ \proba{X=2}}{d\ t} & = & \proba{X=2}\times r_t + \proba{X=5}\times r_l - \proba{X=2}\times 2 \times r_s \proba{X=2} \times 2 \times r_b 
\\ && + \proba{X=11} \times r_f + \proba{X=1} \times 2\times r_t \\
\frac{d\ \proba{X=3}}{d\ t} & = & \proba{X=6} \times r_l - \proba{X=3}\times 2 \times r_s - \proba{X=3} \times 2 \times r_b \\
&& + \proba{X=12} \times r_f + \proba{X=2} \times r_t \\
\frac{d\ \proba{X\subset\{1,2,3\}}}{d\ t} &=&  - 2 \times r_s \times (\proba{X=2}+\proba{X=3}) \\ 
&& - 2 \times r_b \times (\proba{X=1}+\proba{X=2}+\proba{X=3}) \\ 
&& + r_f \times (\proba{X=10}+\proba{X=11}+\proba{X=12}) \\ && 
+ r_l \times (\proba{4}+\proba{5}+\proba{6})
\end{eqnarray*}
Assuming that the servers are saturated and the clients' queue is unlikely to be empty; i.e. $\proba{X=1} \approx 0$, we can transform the equations above into: 
\begin{eqnarray*}
\frac{d\ \proba{X\subset\{1,2,3\}}}{d\ t} &=&  - 2 \times r_s \times (\proba{X=1} + \proba{X=2}+\proba{X=3} ) \\ 
&& - 2 \times r_b \times (\proba{X=1}+\proba{X=2}+\proba{X=3}) \\ 
&& + r_f \times (\proba{X=10}+\proba{X=11}+\proba{X=12}) \\ 
&& + r_l \times (\proba{4}+\proba{5}+\proba{6})+ \prob{6}) \\
&=& -2 \times r_s \times \proba{X\subset\{1,2,3\}} -2 \times r_b \times \proba{X\subset\{1,2,3\}}\\	
&& + r_f \times \proba{X\subset\{10,11,12\}}  + r_l \times \proba{X\subset\{4,5,6\}} 
\end{eqnarray*}
The probability of being in the sub-chain $\{1,2,3\}$ is now expressed in terms of the probability of the other sub-chains. Similar expressions can be calculated for those as well. 
\end{exmp}

\subsubsection{Comparing the Approaches for Deriving the Aggregate Equations}

For a large-scale PEPA model which satisfies Condition \ref{}, we offered two approaches for calculating the corresponding marginal probability distributions. According to the first approach, initially, the aggregated CTMC is constructed and then the aggregate ODEs leading to the marginal distributions are generated. According to the second one, such aggregated ODEs are directly generated by converting the model\rq{}s original C-K equations. Indeed, the two routes lead exactly to the same equations since each sub-chain, to whose probability is referred to when converting C-K equations, is presented as a single state in the aggregate CTMC and this CTMC is faithful in capturing the probability flows into and out of the sub-chains (recall that each sub-chain can be identified by the configuration it captures for the the small groups). However, it should be noted that the cost of deriving the aggregate ODEs and deriving the marginal distributions through using the aggregated CTMC is orders of magnitude smaller than deriving them from the C-K equations as in the former case, one avoids the construction of the large system of C-K equations. 


% this is two verbose
%Consider a large-scale PEPA model which satisfies the aggregation conditions. This suggests that the model\rq{}s CTMC inherently encompasses the structural properties shown in Section \ref{sec:ctmcstructure}. Assuming that the small populations are under heavy load, i.e. the probability of the model being in its boundary states is nearly zero, one can use the model\rq{}s underlying C-K equations and derive a new set of approximate aggregate ODEs. In this set, the probability evolutions are captured only with respect to the sub-chains and the probability information for the individual states is lost. 

%Having the same assumptions about the model, one can take a different route for deriving the aggregate ODEs. Using the reduction rules and count-oriented semantics, one first derives the system\rq{}s aggregate CTMC. This CTMC only captures the state of the instances within the model\rq{}s small groups. Then, using the algorithm shown in Section \ref{equationAlgorithm}, the aggregate ODEs can be constructed. The two routes lead exactly to the same equations since each sub-chain, to whose probability is referred to in C-K equations, is presented as a single state in the aggregate CTMC and this CTMC is faithful in capturing the probability flows into and out of the sub-chains (recall that each sub-chain can be identified by the configuration it captures for the the small groups). However, it should be noted that the cost of deriving the aggregate ODEs through using the aggregated CTMC is orders of magnitude smaller than deriving them from the C-K equations as in the former case, one avoids the construction of the large system of C-K equations. 

In the next section, we consider an experiment where the accuracy of the approximate aggregate ODEs is investigated.


==> CheckingTheAccuracyFinalExperiments/Gnuplots/Outputs/Cr.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(726,1518){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(726,2332){\makebox(0,0)[r]{\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(726,3147){\makebox(0,0)[r]{\strut{} 0.6}}%
      \csname LTb\endcsname%
      \put(726,3961){\makebox(0,0)[r]{\strut{} 0.8}}%
      \csname LTb\endcsname%
      \put(726,4775){\makebox(0,0)[r]{\strut{} 1}}%
      \csname LTb\endcsname%
      \put(858,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1707,484){\makebox(0,0){\strut{} 200}}%
      \csname LTb\endcsname%
      \put(2557,484){\makebox(0,0){\strut{} 400}}%
      \csname LTb\endcsname%
      \put(3406,484){\makebox(0,0){\strut{} 600}}%
      \csname LTb\endcsname%
      \put(4255,484){\makebox(0,0){\strut{} 800}}%
      \csname LTb\endcsname%
      \put(5104,484){\makebox(0,0){\strut{} 1000}}%
      \csname LTb\endcsname%
      \put(5954,484){\makebox(0,0){\strut{} 1200}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} 1400}}%
      \put(3830,154){\makebox(0,0){\strut{}Time}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}$\lll{\proba{Cr = 0}}$ - \textbf{first case}}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}$\lll{\proba{Cr = 0}}$ - \textbf{second case}}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}$\lll{\proba{Cr = 0}}$ - \textbf{third case}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./Outputs/Cr}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> CheckingTheAccuracyFinalExperiments/Gnuplots/Outputs/firstCase_AbstractProbability.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(726,1518){\makebox(0,0)[r]{\strut{} 0.1}}%
      \csname LTb\endcsname%
      \put(726,2332){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(726,3147){\makebox(0,0)[r]{\strut{} 0.3}}%
      \csname LTb\endcsname%
      \put(726,3961){\makebox(0,0)[r]{\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(726,4775){\makebox(0,0)[r]{\strut{} 0.5}}%
      \csname LTb\endcsname%
      \put(858,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1707,484){\makebox(0,0){\strut{} 200}}%
      \csname LTb\endcsname%
      \put(2557,484){\makebox(0,0){\strut{} 400}}%
      \csname LTb\endcsname%
      \put(3406,484){\makebox(0,0){\strut{} 600}}%
      \csname LTb\endcsname%
      \put(4255,484){\makebox(0,0){\strut{} 800}}%
      \csname LTb\endcsname%
      \put(5104,484){\makebox(0,0){\strut{} 1000}}%
      \csname LTb\endcsname%
      \put(5954,484){\makebox(0,0){\strut{} 1200}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} 1400}}%
      \put(3830,154){\makebox(0,0){\strut{}Time}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3905,4602){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{1}} $}}%
      \csname LTb\endcsname%
      \put(3905,4382){\makebox(0,0)[r]{\strut{}$\proba{Z_{a} \subset E^{1}}$}}%
      \csname LTb\endcsname%
      \put(3905,4162){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{2}}$}}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}$\proba{Z_a \subset E^{2}}$}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{5}}$}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}$\proba{Z_a \subset E^{5}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./Outputs/firstCase_AbstractProbability}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> CheckingTheAccuracyFinalExperiments/Gnuplots/Outputs/firstCase_StateProbability.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(858,1722){\makebox(0,0)[r]{\strut{} 0.05}}%
      \csname LTb\endcsname%
      \put(858,2740){\makebox(0,0)[r]{\strut{} 0.1}}%
      \csname LTb\endcsname%
      \put(858,3757){\makebox(0,0)[r]{\strut{} 0.15}}%
      \csname LTb\endcsname%
      \put(858,4775){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1820,484){\makebox(0,0){\strut{} 200}}%
      \csname LTb\endcsname%
      \put(2651,484){\makebox(0,0){\strut{} 400}}%
      \csname LTb\endcsname%
      \put(3481,484){\makebox(0,0){\strut{} 600}}%
      \csname LTb\endcsname%
      \put(4312,484){\makebox(0,0){\strut{} 800}}%
      \csname LTb\endcsname%
      \put(5142,484){\makebox(0,0){\strut{} 1000}}%
      \csname LTb\endcsname%
      \put(5973,484){\makebox(0,0){\strut{} 1200}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} 1400}}%
      \put(3896,154){\makebox(0,0){\strut{}Time}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3641,4602){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{005}}}$}}%
      \csname LTb\endcsname%
      \put(3641,4382){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_{a}=005}}$}}%
      \csname LTb\endcsname%
      \put(3641,4162){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{311}}}$}}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_a=311}}$}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{500}}}$}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_a =500}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./Outputs/firstCase_StateProbability}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> CheckingTheAccuracyFinalExperiments/Gnuplots/Outputs/secondCase_AbstractProbability.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(726,1518){\makebox(0,0)[r]{\strut{} 0.1}}%
      \csname LTb\endcsname%
      \put(726,2332){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(726,3147){\makebox(0,0)[r]{\strut{} 0.3}}%
      \csname LTb\endcsname%
      \put(726,3961){\makebox(0,0)[r]{\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(726,4775){\makebox(0,0)[r]{\strut{} 0.5}}%
      \csname LTb\endcsname%
      \put(858,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1707,484){\makebox(0,0){\strut{} 200}}%
      \csname LTb\endcsname%
      \put(2557,484){\makebox(0,0){\strut{} 400}}%
      \csname LTb\endcsname%
      \put(3406,484){\makebox(0,0){\strut{} 600}}%
      \csname LTb\endcsname%
      \put(4255,484){\makebox(0,0){\strut{} 800}}%
      \csname LTb\endcsname%
      \put(5104,484){\makebox(0,0){\strut{} 1000}}%
      \csname LTb\endcsname%
      \put(5954,484){\makebox(0,0){\strut{} 1200}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} 1400}}%
      \put(3830,154){\makebox(0,0){\strut{}Time}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3905,4602){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{1}} $}}%
      \csname LTb\endcsname%
      \put(3905,4382){\makebox(0,0)[r]{\strut{}$\proba{Z_{a} \subset E^{1}}$}}%
      \csname LTb\endcsname%
      \put(3905,4162){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{2}}$}}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}$\proba{Z_a \subset E^{2}}$}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{5}}$}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}$\proba{Z_a \subset E^{5}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./Outputs/secondCase_AbstractProbability}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> CheckingTheAccuracyFinalExperiments/Gnuplots/Outputs/secondCase_StateProbability.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(858,1722){\makebox(0,0)[r]{\strut{} 0.05}}%
      \csname LTb\endcsname%
      \put(858,2740){\makebox(0,0)[r]{\strut{} 0.1}}%
      \csname LTb\endcsname%
      \put(858,3757){\makebox(0,0)[r]{\strut{} 0.15}}%
      \csname LTb\endcsname%
      \put(858,4775){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1820,484){\makebox(0,0){\strut{} 200}}%
      \csname LTb\endcsname%
      \put(2651,484){\makebox(0,0){\strut{} 400}}%
      \csname LTb\endcsname%
      \put(3481,484){\makebox(0,0){\strut{} 600}}%
      \csname LTb\endcsname%
      \put(4312,484){\makebox(0,0){\strut{} 800}}%
      \csname LTb\endcsname%
      \put(5142,484){\makebox(0,0){\strut{} 1000}}%
      \csname LTb\endcsname%
      \put(5973,484){\makebox(0,0){\strut{} 1200}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} 1400}}%
      \put(3896,154){\makebox(0,0){\strut{}Time}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3641,4602){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{500}}}$}}%
      \csname LTb\endcsname%
      \put(3641,4382){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_a=500}}$}}%
      \csname LTb\endcsname%
      \put(3641,4162){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{311}}}$}}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_a=311}}$}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{005}}}$}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_{a}=S_{005}}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./Outputs/secondCase_StateProbability}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> CheckingTheAccuracyFinalExperiments/Gnuplots/Outputs/thirdCase_AbstractProbability.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(726,1518){\makebox(0,0)[r]{\strut{} 0.1}}%
      \csname LTb\endcsname%
      \put(726,2332){\makebox(0,0)[r]{\strut{} 0.2}}%
      \csname LTb\endcsname%
      \put(726,3147){\makebox(0,0)[r]{\strut{} 0.3}}%
      \csname LTb\endcsname%
      \put(726,3961){\makebox(0,0)[r]{\strut{} 0.4}}%
      \csname LTb\endcsname%
      \put(726,4775){\makebox(0,0)[r]{\strut{} 0.5}}%
      \csname LTb\endcsname%
      \put(858,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1707,484){\makebox(0,0){\strut{} 200}}%
      \csname LTb\endcsname%
      \put(2557,484){\makebox(0,0){\strut{} 400}}%
      \csname LTb\endcsname%
      \put(3406,484){\makebox(0,0){\strut{} 600}}%
      \csname LTb\endcsname%
      \put(4255,484){\makebox(0,0){\strut{} 800}}%
      \csname LTb\endcsname%
      \put(5104,484){\makebox(0,0){\strut{} 1000}}%
      \csname LTb\endcsname%
      \put(5954,484){\makebox(0,0){\strut{} 1200}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} 1400}}%
      \put(3830,154){\makebox(0,0){\strut{}Time}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3905,4602){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{1}} $}}%
      \csname LTb\endcsname%
      \put(3905,4382){\makebox(0,0)[r]{\strut{}$\proba{Z_{a} \subset E^{1}}$}}%
      \csname LTb\endcsname%
      \put(3905,4162){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{2}}$}}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}$\proba{Z_a \subset E^{2}}$}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}$\proba{Z \subset E^{5}}$}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}$\proba{Z_a \subset E^{5}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./Outputs/thirdCase_AbstractProbability}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> CheckingTheAccuracyFinalExperiments/Gnuplots/Outputs/thirdCase_StateProbability.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(858,1247){\makebox(0,0)[r]{\strut{} 0.02}}%
      \csname LTb\endcsname%
      \put(858,1790){\makebox(0,0)[r]{\strut{} 0.04}}%
      \csname LTb\endcsname%
      \put(858,2332){\makebox(0,0)[r]{\strut{} 0.06}}%
      \csname LTb\endcsname%
      \put(858,2875){\makebox(0,0)[r]{\strut{} 0.08}}%
      \csname LTb\endcsname%
      \put(858,3418){\makebox(0,0)[r]{\strut{} 0.1}}%
      \csname LTb\endcsname%
      \put(858,3961){\makebox(0,0)[r]{\strut{} 0.12}}%
      \csname LTb\endcsname%
      \put(858,4504){\makebox(0,0)[r]{\strut{} 0.14}}%
      \csname LTb\endcsname%
      \put(990,484){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1820,484){\makebox(0,0){\strut{} 200}}%
      \csname LTb\endcsname%
      \put(2651,484){\makebox(0,0){\strut{} 400}}%
      \csname LTb\endcsname%
      \put(3481,484){\makebox(0,0){\strut{} 600}}%
      \csname LTb\endcsname%
      \put(4312,484){\makebox(0,0){\strut{} 800}}%
      \csname LTb\endcsname%
      \put(5142,484){\makebox(0,0){\strut{} 1000}}%
      \csname LTb\endcsname%
      \put(5973,484){\makebox(0,0){\strut{} 1200}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} 1400}}%
      \put(3896,154){\makebox(0,0){\strut{}Time}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3641,4602){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{500}}}$}}%
      \csname LTb\endcsname%
      \put(3641,4382){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_a=500}}$}}%
      \csname LTb\endcsname%
      \put(3641,4162){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{311}}}$}}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_a=311}}$}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z \subset S_{005}}}$}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}$\lll{\proba{Z_{a}=005}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{./Outputs/thirdCase_StateProbability}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> CheckingTheAccuracyFinalExperiments/Gnuplots/plotScript <==
reset

set terminal epslatex

set datafile separator ","

# point type 1 = '+'
# point type 2 = 'x'
# point type 3 = '+ and x'
# point type 4 = 'box'
# point type 5 = 'filled box'
# point type 6 = 'empty circle'
# point type 7 = 'filled circle'

# styles for the first case

set style line 1 linecolor rgb "#0f0f0f" linetype 1 linewidth 5 pointtype 1 pointsize 4 
set style line 2 linecolor rgb "#0f0f0f" linetype 2 linewidth 5 pointtype 2 pointsize 4 
set style line 3 linecolor rgb "#0f0f0f" linetype 5 linewidth 5 pointtype 3 pointsize 4 

set style line 4 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 2 pointsize 4 
set style line 5 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 5 pointsize 3 
set style line 6 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 7 pointsize 3

# styles for the second case

set style line 21 linecolor rgb "#0f0f0f" linetype 1 linewidth 5 pointtype 1 pointsize 4
set style line 22 linecolor rgb "#0f0f0f" linetype 2 linewidth 5 pointtype 2 pointsize 4
set style line 23 linecolor rgb "#0f0f0f" linetype 5 linewidth 5 pointtype 3 pointsize 4    

set style line 25 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 2 pointsize 4 
set style line 26 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 4 pointsize 3 
set style line 27 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 7 pointsize 3

# styles for the third case

set style line 31 linecolor rgb "#0f0f0f" linetype 1 linewidth 5 pointtype 1 pointsize 4
set style line 32 linecolor rgb "#0f0f0f" linetype 2 linewidth 5 pointtype 2 pointsize 4
set style line 33 linecolor rgb "#0f0f0f" linetype 5 linewidth 5 pointtype 3 pointsize 4    

set style line 35 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 2 pointsize 3 
set style line 36 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 5 pointsize 3 
set style line 37 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 7 pointsize 2


#set style line 7 linecolor rgb "#8b8682" linetype 1 linewidth 6 pointtype 7 pointsize 2 
#set style line 8 linecolor rgb "#8b8682" linetype 1 linewidth 6 pointtype 5 pointsize 2 
#set style line 9 linecolor rgb "#8b8682" linetype 1 linewidth 6 pointtype 2 pointsize 2
#set style line 10 linecolor rgb "#8b8682" linetype 1 linewidth 3 pointtype 5 pointsize 1 
#set style line 11 linecolor rgb "#8b8682" linetype 1 linewidth 3 pointtype 7 pointsize 1


set grid

set xrange [0:1400]
set xlabel "Time"

set key vertical maxrows 3
set key font ",10"

#--------------------------------
# firstCase, state probability
#--------------------------------

set output './Outputs/firstCase_StateProbability.tex'

set yrange [0:0.2]

plot 	"S_005_exact_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{005}}}$" with linespoints ls 4, \
	"S_005_approximate_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z_{a}=005}}$" with line ls 1, \
	"S_311_exact_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{311}}}$" with linespoints ls 5, \
	"S_311_approximate_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=311}}$" with line ls 2, \
	"S_500_exact_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{500}}}$" with linespoints ls 6, \
	"S_500_approximate_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z_a =500}}$" with line ls 3 

#--------------------------------
# firstCase, abstract probability
#--------------------------------

set output './Outputs/firstCase_AbstractProbability.tex'

set yrange [0:0.5]

plot 	"S_1_exact_firstCase.csv" using 1:2 title "$\\proba{Z \\subset E^{1}} $" with linespoints ls 4, \
	"S_1_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_{a} \\subset E^{1}}$" with line ls 1, \
	"S_2_exact_firstCase.csv" using 1:2 title "$\\proba{Z \\subset E^{2}}$" with linespoints ls 5, \
	"S_2_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{2}}$" with line ls 2, \
	"S_5_exact_firstCase.csv" using 1:2 title "$\\proba{Z \\subset E^{5}}$" with linespoints ls 6, \
	"S_5_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{5}}$" with line ls 3 



#--------------------------------
# secondCase, state probability
#--------------------------------

set output './Outputs/secondCase_StateProbability.tex'

set yrange [0:0.2]

plot 	"S_500_exact_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{500}}}$" with linespoints ls 25, \
	"S_500_approximate_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=500}}$" with line ls 21, \
	"S_311_exact_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{311}}}$" with linespoints ls 26, \
	"S_311_approximate_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=311}}$" with line ls 22, \
	"S_005_exact_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{005}}}$" with linespoints ls 27, \
	"S_005_approximate_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z_{a}=S_{005}}}$" with line ls 23


#--------------------------------
# secondCase, abstract probability
#--------------------------------

set output './Outputs/secondCase_AbstractProbability.tex'

set yrange [0:0.5]

plot 	"S_1_exact_secondCase.csv" using 1:2 title "$\\proba{Z \\subset E^{1}} $" with linespoints ls 25, \
	"S_1_approximate_secondCase.csv" using 1:2 title "$\\proba{Z_{a} \\subset E^{1}}$" with line ls 21, \
	"S_2_exact_secondCase.csv" using 1:2 title "$\\proba{Z \\subset E^{2}}$" with linespoints ls 26, \
	"S_2_approximate_secondCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{2}}$" with line ls 22, \
	"S_5_exact_secondCase.csv" using 1:2 title "$\\proba{Z \\subset E^{5}}$" with linespoints ls 27, \
	"S_5_approximate_secondCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{5}}$" with line ls 23 


#--------------------------------
# ThirdCase, state probability
#--------------------------------

set output './Outputs/thirdCase_StateProbability.tex'

set yrange [0:0.15]

plot 	"S_500_exact_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{500}}}$" with linespoints ls 35, \
	"S_500_approximate_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=500}}$" with line ls 31,\
	"S_311_exact_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{311}}}$" with linespoints ls 36, \
	"S_311_approximate_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=311}}$" with line ls 32, \
	"S_005_exact_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{005}}}$" with linespoints ls 37, \
	"S_005_approximate_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z_{a}=005}}$" with line ls 33


#--------------------------------
# ThirdCase, abstract probability
#--------------------------------

set output './Outputs/thirdCase_AbstractProbability.tex'

set yrange [0:0.5]

plot 	"S_1_exact_thirdCase.csv" using 1:2 title "$\\proba{Z \\subset E^{1}} $" with linespoints ls 35, \
	"S_1_approximate_thirdCase.csv" using 1:2 title "$\\proba{Z_{a} \\subset E^{1}}$" with line ls 31, \
	"S_2_exact_thirdCase.csv" using 1:2 title "$\\proba{Z \\subset E^{2}}$" with linespoints ls 36, \
	"S_2_approximate_thirdCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{2}}$" with line ls 32, \
	"S_5_exact_thirdCase.csv" using 1:2 title "$\\proba{Z \\subset E^{5}}$" with linespoints ls 37, \
	"S_5_approximate_thirdCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{5}}$" with line ls 33 


#--------------------------------
# C_r. The probability of being in boundary states.
#--------------------------------

set style line 12 linecolor rgb "#0f0f0f" linetype 1 linewidth 10 pointtype 1 pointsize 3

set style line 13 linecolor rgb "#0f0f0f" linetype 2 linewidth 7 pointtype 2 pointsize 3

set style line 14 linecolor rgb "#0f0f0f" linetype 6 linewidth 7 pointtype 3 pointsize 3

set output './Outputs/Cr.tex'

set yrange [0:1]

plot 	"C_r_firstCase.csv" using 1:2 title "$\\lll{\\proba{Cr = 0}}$ - \\textbf{first case}" with lines ls 12, \
	"C_r_secondCase.csv" using 1:2 title "$\\lll{\\proba{Cr = 0}}$ - \\textbf{second case}" with lines ls 13, \
	"C_r_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Cr = 0}}$ - \\textbf{third case}" with lines ls 14



==> CheckingTheAccuracyFinalExperiments/Gnuplots/plotScript_ <==
reset

set terminal epslatex

set datafile separator ","

# point type 1 = '+'
# point type 2 = 'x'
# point type 3 = '+ and x'
# point type 4 = 'box'
# point type 5 = 'filled box'
# point type 6 = 'empty circle'
# point type 7 = 'filled circle'

# styles for the first case

set style line 1 linecolor rgb "#0f0f0f" linetype 1 linewidth 5 pointtype 1 pointsize 4 
set style line 2 linecolor rgb "#0f0f0f" linetype 2 linewidth 5 pointtype 2 pointsize 4 
set style line 3 linecolor rgb "#0f0f0f" linetype 5 linewidth 5 pointtype 3 pointsize 4 

set style line 4 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 2 pointsize 4 
set style line 5 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 5 pointsize 3 
set style line 6 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 7 pointsize 3

# styles for the second case

set style line 21 linecolor rgb "#0f0f0f" linetype 1 linewidth 5 pointtype 1 pointsize 4
set style line 22 linecolor rgb "#0f0f0f" linetype 2 linewidth 5 pointtype 2 pointsize 4
set style line 23 linecolor rgb "#0f0f0f" linetype 5 linewidth 5 pointtype 3 pointsize 4    

set style line 25 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 2 pointsize 4 
set style line 26 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 4 pointsize 3 
set style line 27 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 7 pointsize 3

# styles for the third case

set style line 31 linecolor rgb "#0f0f0f" linetype 1 linewidth 5 pointtype 1 pointsize 4
set style line 32 linecolor rgb "#0f0f0f" linetype 2 linewidth 5 pointtype 2 pointsize 4
set style line 33 linecolor rgb "#0f0f0f" linetype 5 linewidth 5 pointtype 3 pointsize 4    

set style line 35 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 2 pointsize 3 
set style line 36 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 5 pointsize 3 
set style line 37 linecolor rgb "#8b8682" linetype 1 linewidth 1 pointtype 7 pointsize 2


#set style line 7 linecolor rgb "#8b8682" linetype 1 linewidth 6 pointtype 7 pointsize 2 
#set style line 8 linecolor rgb "#8b8682" linetype 1 linewidth 6 pointtype 5 pointsize 2 
#set style line 9 linecolor rgb "#8b8682" linetype 1 linewidth 6 pointtype 2 pointsize 2
#set style line 10 linecolor rgb "#8b8682" linetype 1 linewidth 3 pointtype 5 pointsize 1 
#set style line 11 linecolor rgb "#8b8682" linetype 1 linewidth 3 pointtype 7 pointsize 1


set grid

set xrange [0:1400]
set xlabel "Time"

set key vertical maxrows 3
set key font ",10"

#--------------------------------
# firstCase, state probability
#--------------------------------

set output './Outputs/firstCase_StateProbability.tex'

set yrange [0:0.2]

plot 	"S_005_exact_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{005}}}$" with linespoints ls 4, \
	"S_005_approximate_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z_{a}=005}}$" with line ls 1, \
	"S_311_exact_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{311}}}$" with linespoints ls 5, \
	"S_311_approximate_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=311}}$" with line ls 2, \
	"S_500_exact_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{500}}}$" with linespoints ls 6, \
	"S_500_approximate_firstCase.csv" using 1:2 title "$\\lll{\\proba{Z_a =500}}$" with line ls 3 

#--------------------------------
# firstCase, abstract probability
#--------------------------------

set output './Outputs/firstCase_AbstractProbability.tex'

set yrange [0:0.5]

plot 	"S_1_exact_firstCase.csv" using 1:2 title "$\\proba{Z \\subset E^{1}} $" with linespoints ls 4, \
	"S_1_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_{a} \\subset E^{1}}$" with line ls 1, \
	"S_2_exact_firstCase.csv" using 1:2 title "$\\proba{Z \\subset E^{2}}$" with linespoints ls 5, \
	"S_2_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{2}}$" with line ls 2, \
	"S_5_exact_firstCase.csv" using 1:2 title "$\\proba{Z \\subset E^{5}}$" with linespoints ls 6, \
	"S_5_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{5}}$" with line ls 3 



#--------------------------------
# secondCase, state probability
#--------------------------------

set output './Outputs/secondCase_StateProbability.tex'

set yrange [0:0.2]

plot 	"S_500_exact_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{500}}}$" with linespoints ls 25, \
	"S_500_approximate_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=500}}$" with line ls 21, \
	"S_311_exact_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{311}}}$" with linespoints ls 26, \
	"S_311_approximate_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=311}}$" with line ls 22, \
	"S_005_exact_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{005}}}$" with linespoints ls 27, \
	"S_005_approximate_secondCase.csv" using 1:2 title "$\\lll{\\proba{Z_{a}=S_{005}}}$" with line ls 23


#--------------------------------
# secondCase, abstract probability
#--------------------------------

set output './Outputs/secondCase_AbstractProbability.tex'

set yrange [0:0.5]

plot 	"S_1_exact_secondCase.csv" using 1:2 title "$\\proba{Z \\subset E^{1}} $" with linespoints ls 25, \
	"S_1_approximate_secondCase.csv" using 1:2 title "$\\proba{Z_{a} \\subset E^{1}}$" with line ls 21, \
	"S_2_exact_secondCase.csv" using 1:2 title "$\\proba{Z \\subset E^{2}}$" with linespoints ls 26, \
	"S_2_approximate_secondCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{2}}$" with line ls 22, \
	"S_5_exact_secondCase.csv" using 1:2 title "$\\proba{Z \\subset E^{5}}$" with linespoints ls 27, \
	"S_5_approximate_secondCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{5}}$" with line ls 23 


#--------------------------------
# ThirdCase, state probability
#--------------------------------

set output './Outputs/thirdCase_StateProbability.tex'

set yrange [0:0.15]

plot 	"S_500_exact_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{500}}}$" with linespoints ls 35, \
	"S_500_approximate_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=500}}$" with line ls 31,\
	"S_311_exact_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{311}}}$" with linespoints ls 36, \
	"S_311_approximate_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z_a=311}}$" with line ls 32, \
	"S_005_exact_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z \\subset S_{005}}}$" with linespoints ls 37, \
	"S_005_approximate_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Z_{a}=005}}$" with line ls 33


#--------------------------------
# ThirdCase, abstract probability
#--------------------------------

set output './Outputs/thirdCase_AbstractProbability.tex'

set yrange [0:0.5]

plot 	"S_1_exact_thirdCase.csv" using 1:2 title "$\\proba{Z \\subset E^{1}} $" with linespoints ls 35, \
	"S_1_approximate_thirdCase.csv" using 1:2 title "$\\proba{Z_{a} \\subset E^{1}}$" with line ls 31, \
	"S_2_exact_thirdCase.csv" using 1:2 title "$\\proba{Z \\subset E^{2}}$" with linespoints ls 36, \
	"S_2_approximate_thirdCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{2}}$" with line ls 32, \
	"S_5_exact_thirdCase.csv" using 1:2 title "$\\proba{Z \\subset E^{5}}$" with linespoints ls 37, \
	"S_5_approximate_thirdCase.csv" using 1:2 title "$\\proba{Z_a \\subset E^{5}}$" with line ls 33 


#--------------------------------
# C_r. The probability of being in boundary states.
#--------------------------------

set style line 12 linecolor rgb "#0f0f0f" linetype 1 linewidth 10 pointtype 1 pointsize 3

set style line 13 linecolor rgb "#0f0f0f" linetype 2 linewidth 7 pointtype 2 pointsize 3

set style line 14 linecolor rgb "#0f0f0f" linetype 6 linewidth 7 pointtype 3 pointsize 3

set output './Outputs/Cr.tex'

set yrange [0:1]

plot 	"C_r_firstCase.csv" using 1:2 title "$\\lll{\\proba{Cr = 0}}$ - \\textbf{first case}" with lines ls 12, \
	"C_r_secondCase.csv" using 1:2 title "$\\lll{\\proba{Cr = 0}}$ - \\textbf{second case}" with lines ls 13, \
	"C_r_thirdCase.csv" using 1:2 title "$\\lll{\\proba{Cr = 0}}$ - \\textbf{third case}" with lines ls 14



==> CheckingTheAccuracyFinalExperiments/Gnuplots/plotStateProbabilities_ <==
reset

set terminal epslatex

set datafile separator ","

# point type 1 = '+'
# point type 2 = 'x'
# point type 3 = '+ and x'
# point type 4 = 'box'
# point type 5 = 'filled box'
# point type 6 = 'empty circle'
# point type 7 = 'filled circle'

set style line 1 linecolor rgb "#0f0f0f" linetype 1 linewidth 5 pointtype 1 pointsize 4 
set style line 2 linecolor rgb "#0f0f0f" linetype 2 linewidth 5 pointtype 2 pointsize 4 
set style line 3 linecolor rgb "#0f0f0f" linetype 5 linewidth 5 pointtype 3 pointsize 4 
set style line 4 linecolor rgb "#8b8682" linetype 1 linewidth 12 pointtype 2 pointsize 2 
set style line 5 linecolor rgb "#8b8682" linetype 1 linewidth 12 pointtype 4 pointsize 1 
set style line 6 linecolor rgb "#8b8682" linetype 1 linewidth 12 pointtype 7 pointsize 2 

set grid

set xrange [0:1400]
set xlabel "Time"

#--------------------------------
# firstCase, state probability
#--------------------------------

set output 'firstCase_StateProbability.tex'

set yrange [0:0.3]

plot 	"S_005_exact_firstCase.csv" using 1:2 title "$\\proba{Z=S_{005}} $" with linespoints ls 4, \
	"S_005_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_{a}=S_{005}}$" with line ls 1, \
	"S_311_exact_firstCase.csv" using 1:2 title "$\\proba{Z=S_{311}}$" with linespoints ls 5, \
	"S_311_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_a=S_{311}}$" with line ls 2, \
	"S_500_exact_firstCase.csv" using 1:2 title "$\\proba{Z=S_{500}}$" with linespoints ls 6, \
	"S_500_approximate_firstCase.csv" using 1:2 title "$\\proba{Z_a=S_{500}}$" with line ls 3 


#--------------------------------
# firstCase, abstract probability
#--------------------------------

set output 'firstCase_AbstractProbability.tex'

set yrange [0:1]








==> CheckingTheAccuracyFinalExperiments/plotStateProbabilities_ <==
reset

set terminal epslatex 

setxrange [-3,3]
setyrange [-1,1]

set label 1 at -2, 0.5 "$erf(x) = \\frac{2}{\\sqrt{\\pi}}\\int_0^x\\, dt e^{-t^2}$" centre

set output 'errorf.tex'

plot erf(x)


==> Conclusion/conclusion.tex <==
\section{Conclusion}
\label{conclusion}
In this paper we considered a sub-class of large-scale PEPA models. 
These are models each consisting of groups with non-uniform sizes; the models consist of one or more small groups cooperating with some large ones. 
These models reflect the situation in many of the existing communication networks where a small population of resources are used by a rather larger population of resource users.
% As examples, consider a client-server system where a large number of client requests are processed by a small number of servers or a number of links in the Internet backbone which deal with millions of packets. 
%When analysing a model which resides in this sub-class, one might aim specifically at building the model's complete CTMC, which is usually of a very large size, and then use that as the basis of probability  investigations. 
We showed that if the model satisfies two conditions, then, in the analysis phase, an approximate aggregation step would be possible and the result, i.e. the aggregated CTMC, would be a useful tool for efficient derivation of  certain performance metrics. 
These are the conditions. First, the rate of all cooperation between the model's small groups and large ones should be controlled and determined by the small groups only. 
Second, as the model executes, it ought to be unlikely for it to experience its boundary states, i.e. the ones where the small groups are blocked while waiting for the cooperation with the large groups. 
We showed that the second condition is in practice, a realistic one and this guarantees the accuracy of our approximation. 
In this paper,  we proposed an algorithm which, for a conforming model to our conditions, directly derives its aggregated CTMC without constructing the model's original CTMC. 
The aggregated CTMC captures, in a detailed manner, the dynamics of the model's small groups and be used to derive an approximate marginal probability distribution over those groups in the model. 
% It, however, abstracts away from the dynamics of the model's large groups.
Calculating such a distribution using the aggregated CTMC is orders of magnitude faster than when the same distribution is derived from the analysis of the complete CTMC. 

\subsection*{FutureWork}

For a conforming model, the primary use described for its aggregated CTMC is to study the behaviour of the model's small groups. 
However, the aggregated CTMC,  inherently being a compact representative of the model's original CTMC, can be used in more directions. 
When analysing a given large-scale model, depending on the features exhibited by the model's underlying CTMC, different analysis methods might be chosen. 
Detecting whether or not this complete CTMC contains certain features is usually computationally expensive. 
%In fact, the complexity of this task can be proportional to that of the complete analysis itself. 
Our previous experiments show that the aggregation step is capable of preserving \emph{some} (if not all) of the important features exhibited by the complete CTMC. 
Therefore, when detecting these features, instead of considering such large CTMCs, the modeller can search for them in the aggregated versions. 

We will pursue this approach with respect to two specific features: \emph{time scale decomposability} (TSD) and the existence of \emph{rare events}. 
%With respect to TSD, we investigate whether the TSDs observed in a model's aggregated CTMC are any potential source for TSDs in the model's original CTMC. 
Our preliminary experiments suggest that when the dynamics of the small groups, i.e. the aggregated CTMC, exhibits TSD, then under certain conditions, these will also be observable in the original CTMC.  Therefore, one way to detect TSDs in the latter, is to investigate the feature at the level of the aggregated CTMC, as this is a potential source.
A similar conjecture can be formed for the existence of rare events. We intend to investigate whether the rare events detected by the analysis of the aggregated CTMC would also be observable at the higher level.
Our aim is to develop algorithms which considers the model's aggregated CTMC and inform the modeller about the potential existence of important features in the model's original CTMC. 
This helps the modeller to make informed decisions when trying to choose the right method for the analysis of the complete CTMC. 


==> Discussion/discussion.tex <==
\section{Discussion}

\subsection{Realistic Assumption About Boundary States}
% probability of experiencing boundary states.
% boundary states -- can be checked while system in running.
The model needs to exhibit two properties in order for the aggregation scheme to be applicable. 
First, it should satisfy the aggregation Condition \ref{aggregationCondition}. This can be checked through a \emph{syntactic} analysis of the model. 
Second, while \emph{in execution}, the model should rarely experience its boundary states. 
This condition cannot be checked by the syntactic analysis. 
The knowledge on whether the system experiences its boundary states with a negligible probability or not, needs to be supplied either by the domain experts\footnote{I suggest that I stop the sentence right here.}, by monitoring the real system from which the model is constructed or by looking at real systems with similar performance profiles to the one which is being modelled.

Usually, a large scale communication system can be considered to consist of two types of entity; a small population of resources and a rather larger population of resource users. 
When building the system, the design goal would be to satisfy the defined performance agreements with the minimum acquisition of resources; the procurement and maintenance of resources are usually costly. An undesirable scenario is to satisfy the performance requirement by over-provisioning the resources. This leads to resource under-utilisation. 
Another unsatisfactory scenario is not to employ adequate resources. 
Poor performance, below the requirements, is the consequence. 
Having in mind this trade-off between the system performance and resource supply, the designers usually add to the system's resources to the degree that a defined performance profile is reached without incurring resource under-utilisation. 

In the making of a majority of the existing large-scale systems, the above principle has been respected. 
The resources, which are tuned to provide acceptable performance profiles, are usually under heavy contention. 
In most cases, there is competition among the users over using such resources. 
As examples, consider  servers in a realistic client-server system which process client requests at a high rate or the routers in the Internet backbone dealing with a continuous stream of packets.
In these systems, it is highly unlikely for the resources to be blocked by the lack of demand from the users. That is, the probability of being in the boundary states, is nearly zero. 
This suggest that the assumption made by our aggregation scheme on the negligence of the probability of being in such states is not unrealistic. Therefore, we conclude that our method can safely be used in modelling a large number of computer systems, specially, for studying the dynamics of their resources.

%
%In a communication system, usually, the resources of different types form a small population which is accessed by a rather larger population of resource users. These resources are usually under heavy contention and in most cases, the users compete for accessing them. This suggest that at all times, the demand on the side of the users is unlikely to be suspended and hence, the resources rarely experience their blocked states. In such cases, Our aggregation method is useful for efficient performance analysis of the resources. 


\subsection{Usefulness of the Method}

% studying the behaviour of the small populations
\subsubsection{Behaviour of the Small Groups}

% aggregated CTMC, a more compact representation of the Complete CTMC
\subsubsection{Aggregated CTMC, a More Compact Representation of the Complete CTMC}



==> Introduction/introduction.tex <==
\section{Introduction}

% what is PEPA.

Performance Evaluation Process Algebra (PEPA) is a compositional high level language suitable for building formal models of stochastic systems \cite{Hillston:1996}. In order to build the model of a system, first the behaviours of constituent sequential components are defined and then these components are composed to form the system's complete description. The behaviour of each component is defined in terms of the local states it experiences and the actions it undertakes. The composition expresses how the components cooperate when they are put together. 
%Having build the model, the modeller analyses it in order to obtain his performance measures of interest. 
% what are large scale models? 
% say that these models are frequently seen. 
In this paper, we consider a \emph{sub-class} of \emph{large-scale} PEPA models. 
In general, a large-scale PEPA model is one in which there exist one or more components which are instantiated many times to form large populations.
In these models, the interaction between two individual components can be seen at a wider context, that is, the interaction between the corresponding populations. 
Of all large-scale models, the particular sub-class we focus on consists of models where the component populations are of non-uniform sizes. 
In a conforming model, while some components appear in large populations, there still exist some components whose populations are relatively small. 
%The distinctive feature of these models is that they include the interaction of one or more large populations with one or more small populations.
The models in this sub-class reflect the situation in many existing computer and communication networks. 
Assuming that they consist of some \emph{resources} and also some \emph{resource users}, it is the usually the case that the users appear in large populations and are serviced by a relatively smaller population of the resources.  

% numerical vectors
% joint probability distribution. 
Usually, during the analysis phase of a large-scale model and in particular, when building its state space, we are content to abstract away from the behaviour of individual components and focus on the evolution of the populations.
This means that in the state space, we no longer track the local state of each distinct individual component. 
In contrast, at any time, one distribution is constructed for each population and the state of the system is formed when these distributions are put together.
For a given population, its distribution records how the the instances within that population are distributed across the local states possible for those instances. 
The mathematical apparatus used for capturing each state of the system is a numerical vector.
The coordinates in this vector are used for recording the aforementioned distributions. 
The complete state space of the system can be constructed by considering the evolution of this numerical vector. 
The state space can be regarded as a CTMC to which a joint probability distribution can be associated. 
Generally, deriving the full distribution or some related measures (mean, variance, etc.) would be the goal of analysing the model.
%The analysis of this CTMC would result in a joint probability distribution over the populations of the model. 

% what is the problem? 
% what is missing from the spectrum of analysis methods? 
There exists a spectrum of analysis methods which can theoretically be used for the analysis of the large-scale PEPA models in our sub-class. 
At one extreme, the rigorous analysis method aims to first, construct the model's CTMC in a complete form and then, obtain the associated joint probability distribution in full. 
Where possible, this method provides fine-grained information about the model's behaviour, including all aspects of its stochastic behaviour.
% i.e. the complete set of states experienced and the probability of being in each one of them. 
However, for models in our sub-class, due to the problem of state space explosion, such an analysis approach is computationally expensive or even infeasible.  
At the other end of the spectrum, we have the fluid flow analysis. 
This method, instead of finding the CTMC's full joint probability distribution, helps the modeller to derive the distribution's first few moments.
These moments then provide the basis for making judgements about the system's performance. 
The fluid flow analysis has been shown to be useful, specifically,  for models with uniform and large populations.  
However, applying the method on models which belong to our sub-class, might not be sufficient when analysing them. 
As shown in \cite{dontGoWith}, for these models, the fluid flow moments might be too abstract or crude to reflect the system's full distribution (e.g. the distribution might be heavy tail or multi-modal). 
In these situations, the fluid flow analysis is potentially insufficient as its output, i.e. the moments, might not reveal certain important properties about the system's stochastic behaviour. 
%For example, the worst-case scenarios are usually not realised by looking only at the model's first few behavioural moments (mean, variance, etc.). 

Having observed the problems associated with these methods for the analysis of models in our sub-class, we developed a new method particularly tailored for their analysis.
Our method is based on an \emph{approximate} state space \emph{aggregation} and the information it reveals about an input model's complete probability distribution is more detailed and fine-grained than the fluid flow moments. 
At the same time, it avoids constructing the model's very large CTMC.
For a large-scale model in this sub-class, the aggregation is possible only if the model satisfies an aggregation condition. 
This condition is a syntactic one and can be checked by a quick analysis of the model's description. 
For a conforming model, our method first produces an approximate aggregated CTMC. 
Such a CTMC can be regarded as a compact representation of the model's very large one and it is useful for derivation of certain performance measures. 
%This will shown to be useful for deriving certain performance metrics. 
In particular, in the second phase, our method uses it to derive a marginal probability distribution over the small populations in the model. 
%On a model, our method is applicable only when the model in the sub-class satisfies the condition that the interactions between the small populations and the large ones are controlled by the small populations (discussed in detail in Section \ref{condition}). This condition can be checked syntactically on the model. 
%The aggregated CTMC is smaller than the original CTMC and its analysis incurs less computational cost.
The same distribution could have been derived by a computationally expensive analysis of the complete CTMC. However, as the size of the aggregated CTMC is orders of magnitude smaller, our method derives it significantly faster. 
%The output of our method for an input model is a marginal distribution over the model's small populations. 
We checked the usefulness and accuracy of our method in the context of a client-server system. where the requests of a relatively large number of clients are dealt with by a smaller population of servers. 
In this case, the method outputs an accurate marginal distribution which captures the dynamics of the servers. 
This distribution, which can be derived efficiently, is valuable for deriving important performance metrics about the system, such as the throughput distribution, the probability of being in failure modes, etc.  

The paper follows this structure: in Section \ref{preliminaries}, we will introduce the PEPA syntax and state space representation technique used when dealing with a large-scale PEPA model. Section \ref{condition} formally introduces the sub-class, illustrates the syntactic condition checked before applying the approximate aggregation and explains the source of error. Sections \ref{aggregationAlgorithSection} and \ref{calculatingMarginalDistributionSection} show the steps of the aggregation method and the way the associated marginal probability distributions are derived. In Section \ref{checkingTheAccuracy} we investigate the accuracy of the method in the context of an example. The related work is presented in Section \ref{relatedWork} and finally, in Section \ref{conclusion} we conclude and describe how we plan to expand the method in our future research. 




==> Preliminaries/preliminaries.tex <==
\section{Preliminaries}
\label{preliminaries}
PEPA provides the following combinators for model construction\footnote{The combinator $Hiding$ is not used in this paper.}: 

\begin{description}
\item[Prefix]$(\alpha,r).P$ : this denotes a sequential process (or component) which undertakes \emph{activity} $(\alpha,r)$ and then follows the behaviour associated with component $P$. The first element, $\alpha$, is the activity's \emph{action type} and the second, $r$, is the parameter of an exponentially distributed random variable which governs the duration the activity. 
\item[Choice]$P+Q$ : this denotes a process which has the choice of either following the behaviour associated with component $P$ or the behaviour associated with component $Q$. 

\item[Constant]$A\rmdef P$ : this denotes that the behaviour of the process $A$ is the same as the behaviour of process $P$. This combinator is used for defining recursive behaviours.

\item[Cooperation]$P\mysync{L}Q$ : Specifies a process which is composed of two sequential processes who interact by undertaking the shared activities whose action types are specified in a \emph{cooperation set} $L$. A sequential component can independently evolve with respect to activities whose action types are not in the component's cooperation set. However, for a shared activity to be undertaken, all the cooperating components must be ready to enable the activity. PEPA supports multi-way synchronisation; i.e. the number of components evolving through a shared activity can be more than two. The rate of the shared activity is defined to be the \emph{minimum} of the rates at which the cooperating components offer for the activity. This guarantees that no sequential component is required to perform an activity faster than its capability. A \emph{parallel} composition, denoted by $P~||~Q$, describes a cooperation where the cooperation set is empty. The syntax sugar $P[n]$ is used to denote the parallel composition of $n$ identical $P$ processes, $P[n] = \underbrace{P~||~P~|| \ldots ~||~P}_{n\ \text{times}}$.

In a cooperation on a shared activity, some components can be defined to participate \emph{passively}. This can represent a situation where some participating components do not control the cooperation rate and they follow whatever rate the \emph{active} components decide for the shared activity. In PEPA, a special symbol, $\top$, is used to denote the rate of the activities undertaken passively, e.g. if the process $P_1$ undertakes $\alpha$ passively and becomes $P_2$, then $P_1 = (\alpha,\top). P_2$. The passive activities of a sequential component  must be shared with at least one active component, or the model is deemed to be incomplete \cite{Hillston:1996}. 
\end{description}
In large-scale PEPA models, some sequential components are instantiated many times to form large groups of instances. The instances in the same group do not cooperate on any activity and the cooperation takes place between instances that belong to different groups. We use the \emph{grouped} PEPA syntax for unambiguous specification of large-scale PEPA models: 
\begin{eqnarray*}
S & = & (\alpha,r). S\  | \ S + S \  | \ C_s \ \ \ \ \ \ \ \ \ \ \ P  =  P \mysync{L} P\  |\  C \\ 
D & = & D \ ||\ D \ | \ P  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ M  =  M \mysync{L} M\  |\  Y\{D\}  
\end{eqnarray*}
Here $S$ represents a \emph{sequential} component (essentially, a state machine) and $P$ a \emph{model} component which is composed of sequential ones. $C$ is a constant which, depending on its definition, represents either a sequential process or a model one and $C_s$ is a constant which stands for a sequential behaviour. This grouped PEPA syntax, which is an augmentation of the PEPA original syntax, helps build a model in which the component instance groups are explicitly shown. This feature will become useful in the analysis phase. Above, $M$ represents a group of instances. To each group, a unique label is assigned, which is represented by $Y$. $D$ represents the \emph{parallel} composition of the instances of a sequential component. These instances constitute a group. In this paper, we restrict ourselves to grouped PEPA models where all groups are strictly \emph{simple}; i.e. each group contains the instances of one sequential component only. The following is an example of such a model.
\begin{exmp} One can capture the dynamics of a client-server system with Model \ref{model1}.
\begin{model}
\begin{eqnarray*}
C_{think} & \rmdef & (think, r_{t}).C_{req}\  \\
C_{req} & \rmdef & (req, r_{c}).C_{think}\ \\  \\
S_{idle} & \rmdef & (req, r_{s}).S_{log} + (brk, r_{b}).S_{broken}\\
S_{log}  & \rmdef & (log, r_l).S_{idle} \   \\ 
S_{broken} & \rmdef & (fix, r_{f}).S_{idle}\\ \\
 CS & \rmdef & Servers~\{\ S_{idle}[2]\ \}  \mysync{\{ req\}} Clients~\{\ C_{think}[2]\ \}
\end{eqnarray*}
\caption{A PEPA model of a client-server system. \label{model1}}
\end{model}

{\bf Description}. In the first part of each model, the behaviours of the sequential processes involved in the system are expressed. For the client-server system, the behaviour of a client and a server are defined. The behaviour of each client (the first two lines of the model) follows this cycle: the client does some independent thinking with rate $r_t$. When finished, it changes its state to $C_{req}$. Here, the client is waiting to cooperate with a server on a request, a $req$ activity. Upon doing so, it returns to the thinking state. The rate at which a client is capable of undertaking $req$ is $r_c$. A server (the next three lines) has the following cycle: the initial state of a server is $S_{idle}$. In this state, it offers the shared activity of type $req$ to a waiting client and transitions into $S_{log}$. The server is capable of performing $req$ with rate $r_s$. When a server's logging finishes, which happens with rate $r_l$, it returns to the idle state. The model captures the failures of servers too. An idle server might break down, with rate $r_b$ and enter into state $S_{broken}$. A broken server gets fixed with rate $r_f$ and consequently, becomes available for service again. 

The last line of the model is called the \emph{system equation} (corresponding to $M$ in the grammar) where the model is compositionally constructed. This specifies the whole model in terms of how the sequential components get instantiated, their initial states, their groupings and the cooperation pattern between the sequential components as well as between the groups. Here, the model is initialised with two instances of servers being idle and two instances of clients thinking. The servers are in group $Servers$ and the group of the clients is labelled $Clients$. The cooperation set specifies that the instances in group $Servers$ synchronise on $req$ activities with instances in group $Clients$. Also, we know that there is no synchronisation between the instances of servers or clients within their respective groups (the last property is a direct result of the grouped PEPA grammar that it disallows synchronisations inside the groups). 

PEPA original semantics \cite{Hillston:1996} have been augmented with additional structured rules to build grouped PEPA semantics which for a given model, constructs its underlying transition relation. For details, refer to \cite{Hayden:2010}. Here we propose some definitions, based on those in \cite{Hillston:1996,Hayden:2010}, particularly tailored for our purposes.
%Fig. \ref{clientServerSystem} shows the behaviour associated with the client component type and the behaviour associated with the server component type in terms of the states experienced and the actions which can be undertaken. 

%\begin{figure}[]
%        \centering
%        \begin{subfigure}[b]{0.5\textwidth}
%                \centering
%                \includegraphics[width=\textwidth]{./graphs/ServerBehaviour}
%                \caption{the behaviour of the servers shown as a state machine}
%                \label{fig:serverBehaviour}
%        \end{subfigure}%
%        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
%          %(or a blank line to force the subfigure onto a new line)
%        \begin{subfigure}[b]{0.5\textwidth}
%                \centering
%                \includegraphics[width=\textwidth]{./graphs/ClientBehaviour}
%                \caption{the behaviour of a client shown as a state machine}
%                \label{fig:client}
%        \end{subfigure}
%        \caption{the components of a client-server system}\label{clientServerSystem}
%\end{figure}
\end{exmp}

%Grouped PEPA has been equipped with a structured operational semantics which, given a PEPA model, generates its underlying CTMC. Questions regarding the performance of the system can then be answered by analysing the model's CTMC either for the equilibrium or the transient behaviour. Fig. \ref{fig:pepaSOS} shows the PEPA structured operational semantics. 

%Here you should put the G-PEPA structured operational semantics.
%\input{pepaSOS}

% For components which appear in large populations, understanding their emergent behaviour is more important than understanding how a single tagged instance evolves. On the other hand, for a component who instance population is still small, it might still be reasonable to observe distinctively the states an instance goes through.  

% assume that here I have explained the idea of state space representation informally and that the reader knows that we are using counters which capture the distribution of the population across different states. 

% defintions borrowed from Prof. Hillston's PhD thesis and Richard's paper. 

For a grouped PEPA model $\mathbb{M}$, let $\group{\mathbb{M}}$ denote the set of group labels in $\mathbb{M}$. For the client-server model, $\group{CS} = \{Servers,Clients\}$ and in general $\group{\mathbb{M}}=\{H_1,H_2,\ldots,H_i,\ldots, H_{N^{h}_\mathbb{M}}\}$ assuming that there are $N^{h}_{\mathbb{M}}$ groups in $\mathbb{M}$. $\group{\mathbb{M}}$ can be recursively calculated: 
\begin{eqnarray}
\group{\mathbb{M}} & = & \left\{			\begin{array}{cl}
									{M_1} \cup {M_2} &\ \ \ \  \  \text{if} \ \ \   \mathbb{M} = M_1 \mysync{L} M_2   \\
									Y & \ \ \ \  \  \text{if} \ \ \   \mathbb{M} = Y\{D\}
								\end{array} \right. 
\end{eqnarray}

Let $\mathcal{C}_{\mathbb{M}} = \{C_1,C_2,\ldots, C_{N^{c}_\mathbb{M}}\}$ be the set of sequential processes (or components) defined in the model (we are assuming in $\mathbb{M}$,  $N^{c}_{\mathbb{M}}$ distinct sequential processes are defined). Given that all groups in $\mathbb{M}$ are simple, i.e. each group consists of the instances of one sequential component only, we can construct the function $sc(H): \group{\mathbb{M}} \rightarrow \mathcal{C}$ which relates a group's label to the sequential component whose instances form that group\footnote{sc stands for ``sequential component".}. For example, $sc(Servers) = S_{idle}$. Note that for a sequential process, we assume that it gets represented by its initial state. Constructing this function enables us to easily lift the definitions in \cite{Hillston:1996} for PEPA models up to the context of grouped PEPA models. 

Each instance of a sequential component $C \in \mathcal{C}_{\mathbb{M}}$ visits a set of local states or local derivatives. Let this set be denoted by $ds(C)$ (Def. 3.4.2 in \cite{Hillston:1996}) (e.g. $ds(S_{idle})=\{S_{idle},S_{log},S_{broken}\}$ and $ds(C_{think})=\{C_{req},C_{think}\}$). 
In general, $ds(C_{x})_{C_x \in \mathcal{C}}=\{C_{x,1},C_{x,2},\ldots,C_{x,y}, \ldots, C_{x,N_{C_x}}\}$, assuming that the sequential component $C_x$ experiences $N_{C_x}$ local states. 
Accordingly, we can define $ds^{*}(H)$ to be the set of local states which the instances in the group labelled $H$ experience (e.g. $ds^{*}(Servers) = \{ S_{idle},S_{log},S_{broken} \}$). For a group $H \in \mathcal{G}(\mathbb{M})$:
\[ds^{*}(H)= ds(sc(H)).\] 
%assuming that the instances of sequential component $C_x$ form the group $H_i$ and $C_x$ local states are enumerated as above where $n_x$ is the number of local states which a $C_x$ process visits.

Each local state that a sequential component $C_x \in \mathcal{C}_{\mathbb{M}}$ visits enables some activities. Let $\mathcal{A}ct(C_{x,y})$ where ${{C_{x,y} \in\  ds(C_x)}}$ be the multi-set of activities enabled by a sequential process $C_{x,y}$\footnote{In process algebra, there is no distinction between sequential processes and the local states they visit. The local state $C_{x,y}$ of the sequential process $C_x$ can indeed itself  represent a sequential process exhibiting the behaviour associated with the state $C_{x,y}$ \cite{Hillston:1996}. In this paper, for illustration purposes, the set of local states of each sequential process are represented by a single state chosen for that process.}. (Def. 3.3.3 in \cite{Hillston:1996}). Then, $\stackrel{\rightarrow}{\mathcal{A}ct}(C_{x})$, the set of complete activities undertaken by instances of $C_{x}$, can be defined as: 
\[\stackrel{\rightarrow}{\mathcal{A}ct}(C_{x}) = \bigcup_{C_{x,y} \in ds(C_x)}^{} \mathcal{A}ct\ (C_{x,y})\]
Let $\stackrel{\rightarrow}{\mathcal{A}ct^{*}}(H)$ denote the set of activities enabled by the instances in a group labelled $H$. 
Assuming that the groups are simple, we have:
\[\stackrel{\rightarrow}{\mathcal{A}ct^{*}}(H) = \ \stackrel{\rightarrow}{\mathcal{A}ct}(C_{x})\ \ \\ \ \ \ \ \text{where}\ \ \ \ \ C_x = sc(H). \]
%The reverse function $d_s^{-1}(\cdot)$ takes a local state and outputs the component type to which the local state belongs. For example, $d_s^{-1}(Server_{requesting})=Server$. 
% 
In the client-server system: 
\[\stackrel{\rightarrow}{\mathcal{A}ct^{*}}(Servers)=\{(req,r_s),(log,r_l),((break,r_b),(fix,r_f)\}.\]

For an action type $\alpha$, we define $En(\alpha)$ to be the set of local states which enable an activity of that type. This notion is originally defined in \cite{1595779}. Here we propose  a similar definition based on $\mathcal{A}ct(C_{x,y})$: 
\begin{eqnarray*}
En(\alpha) & = & \bigcup_{C_x\  \in\  \mathcal{C}} En^{\prime}(\alpha,C_x), \\
En^{\prime}(\alpha,C_x) & = & \bigcup_{C_{x,y}\  \in\  ds(C_x)} En^{\prime\prime}(\alpha,C_{x,y}), \\
En^{\prime\prime}(\alpha,C_x,C_{x,y}) &=& \left\{	\begin{array}{ll} 
																				C_{x,y} &\ \ \ \ \ \text{if} \ \ (\alpha,\cdot) \in \mathcal{A}ct(C_{x,y}) \\
																				\{\} &\ \ \ \ \  \text{otherwise.} \\ 	
																			\end{array}\right.
\end{eqnarray*}
$En^{\prime}(\alpha,C_x)$ returns the set of local states in $ds(C_x)$ which enable $\alpha$. $En^{\prime\prime}(\alpha,C_x,C_{x,y})$ works at the level of individual local states; it returns a local state if it enables $\alpha$. 

In the system equation of a model, the operator $\mysync{L}$ is used to put together the model's groups and form cooperations. 
The instances of two groups which are composed are restricted to synchronize on the action types in the associated cooperation set. 
Moreover, these groups can be subjected to further compositions and synchronizations with other groups of the model. 
In such a case, the instances in these two groups will have to respect further synchronization restrictions.
From this point of view, one aspect of a model's system equation is that it introduces a \emph{hierarchy of cooperation} among the model's different groups and assigns to each group, the set of action types the instances in that group need to synchronize on. To clarify, consider the process 
\[( G_1\{\cdot\} \mysync{L^{\prime}} G_2\{\cdot\} ) \mysync{L} ( G_3\{\cdot\} \mysync{L^{\prime\prime}} G_4\{\cdot\} ).  \]

Here $G_1$ and $G_2$ are composed in the context of cooperation on set $L^{\prime}$. 
Similarly, $G_3$ and $G_4$ form a composition as their instances cooperate on actions in set $L^{\prime\prime}$. 
Additionally, these group compositions are again combined to form yet another larger composition; i.e. the cooperation on set $L$. 
Here, the cooperation on set $L^{\prime}$ restricts the instances in groups $G_1$ and $G_2$ and does not affect $G_3$ or $G_4$; the instances in groups $G_3$ and $G_4$ can proceed with activities of action type $\mathcal{A} - L^{\prime}-L$,
%(in particular $ L^{\prime} - (L \cup L ^{\prime\prime}))$,
if enabled, without waiting for instances in the groups $G_1$ and $G_2$ so long as the synchronization on $L^{\prime\prime}$ is respected. 
%In other words, the scope of the cooperation on $L^{\prime}$ includes $G_1$ and $G_2$ and does not include $G_3$ and $G_4$. 
Similarly, the scope of the cooperation on set $L^{\prime\prime}$ includes the groups $G_3$ and $G_4$ and does not include $G_1$ and $G_2$. The scope of the cooperation with set $L$, which is regarded to be at a higher level, includes all groups $G_1$, $G_2$, $G_3$ and $G_4$. 

We formalize the above idea with the notion of the \emph{interface} of a group. For a group $H$ in model $\mo{M}$, $\interface{M}{H}$ denotes the set of action types on which the instances in $H$ are required to synchronize. $\interface{M}{H}$ can be calculated by considering the system equation, in which the group structure is embedded, and using the subsidiary function $\mathcal{J}$; $\interface{M}{H} = \subsid{\mo{M}}{H}{\emptyset}$

\begin{eqnarray*}
\subsid{M}{H}{K} &  = & 	\left \{ 
												\begin{array}{ll}
													K, &  \\ 
												 \ \ \ \ \ \ \ \ \ \text{if}\ \ \  M = Y\{\cdot\} \ \wedge\  Y = H \ \ ,\ \ Y,H \in \group{M}. & \\ \\
													\subsid{M_1}{H}{K \cup L } \cup \subsid{M_2}{H}{K\cup L }, & \\
													 \ \ \ \ \ \ \ \ \ \text{if} \ \ \ M = M_1 \mysync{L} M_2. & \\ \\
													 \subsid{A}{H}{K}, &  \\
													 \ \ \ \ \ \ \ \ \ \text{if}\ \ \ M \rmdef A.  & 												\end{array}
											\right.
\end{eqnarray*}

According to this definition, the interface $\interface{M}{H}$ of group $H$ might contain action types which are not enabled in any of the local states $ds^{*}(H)$. Therefore, we define $\einterface{M}{H}$ to represent the \emph{active} interface of $H$, which contains only the action types in $\interface{M}{H}$ which are enabled in at least one local state in $ds^{*}(H)$. More formally, let $\stackrel{\rightarrow}{\mathcal{A}^{*}}(H) = \{\alpha \ |\ (\alpha,r) \ \in\  \activities{H} \}$ be the set of all action types enabled by $H$. Then: 
\[ \einterface{M}{H} = \interface{M}{H} \ \ \cap\ \ \actions{H}. \]

A related notion concerning the interface of a group is $\coop{M}{H}{\alpha}$; this represents the set of groups in $\mo{M}$ whose instances synchronize on $\alpha$ activities with instances in group $H$. 
In order to formally define $\coop{M}{H}{\alpha}$, let us first define the partial order relation $<^{*}$ on $\mo{M}$'s groups. 
This relation captures the hierarchy of cooperation represented by $\mo{M}$'s system equation. $\subgroup{G_1}{G_2}$, for $G_1$ and $G_2$ each being a composition of groups, means that $G_1$ is composed (or is included) when constructing $G_2$. 
In this case, all the cooperation sets applied on $G_2$ are also enforced on $G_1$. For model $\mo{M}$, the relation $<^{*}$ can be constructed following these rules: 
\begin{eqnarray*}
1.&&  H\{\cdot\}  <^{*}  H\{\cdot\}    \\
2.&&  H\{\cdot\}  <^{*}  {H_1\{\cdot\} \mysync{L} H_2\{\cdot\}}  \ \ \ \ \ \text{if}\ \ \ \ \ \  H=H_1 \vee H=H_2 \\
3.&&  X <^{*}  A  \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ \text{if}\ \ \ \ \ \  A \rmdef X
\end{eqnarray*}
Having constructed $<^{*}$, we can define $\coop{M}{H}{\alpha}$ as follows:
\begin{eqnarray*}
\coop{M}{H}{\alpha} & = & \left\{		\begin{array}{ll}
															\emptyset & \text{if}\ M = H\{\cdot\} \\ \\
															\coop{M_1}{H}{\alpha} \cup \{H_i \in \group{M} \mid H_i\{\cdot\} <^{*}\ M_2\} & \text{if}\ M=M_1 \mysync{L} M_2, \alpha\in L, \\ 
															 & H<^{*} M_1	\\ \\ \\
															\coop{M_2}{H}{\alpha} \cup \{H_i \in \group{M} \mid H_i\{\cdot\} <^{*}\ M_1\} & \text{if}\ M=M_1 \mysync{L} M_2, \alpha\in L, \\ 
															 & H<^{*} M_2	\\ \\ \\
															\coop{M_1}{H}{\alpha} & \text{if}\ M=M_1 \mysync{L} M_2, \alpha\not\in L, \\ 
															 & H<^{*} M_1	\\ \\ \\
															\coop{M_2}{H}{\alpha} & \text{if}\ M=M_1 \mysync{L} M_2, \alpha\not\in L, \\ 
															 & H<^{*} M_2	\\ \\ \\
%															 \emptyset & \text{if}\ M=M_1 \mysync{L} M_2 \wedge \alpha\not\in L \wedge H\{\cdot\} \not<^{*} M_1 \wedge H\{\cdot\} \not<^{*} M_2 \\ \\
															\coop{A}{H}{\alpha} & \text{if}\ M \rmdef A 
														\end{array}\right.
\end{eqnarray*}
The definition is based on the intuition that if, in the synchronization hierarchy, a group composition is required to synchronise on an action set, then all the member groups, which reside in this group composition, are required to synchronise on that action set.

\begin{exmp}
Consider the following system equation:
\[E = \Big(\  (\  H_1\{\cdot\} \mysync{\{\alpha,\beta\}} H_2\{\cdot\}\  )\ \mysync{\{\theta\}} H_3\{\cdot\} \ \Big) \  \mysync{\{\alpha\}} \  (\  H_4\{\cdot\} \mysync{\{\gamma\}} H_5\{\cdot\}\  )  \]
which represents this hierarchy for the groups:

\begin{eqnarray*}
\Tree[
		.$\mysync{\{\alpha\}}$
			 [.$\mysync{\{\theta\}}$ 
					[.$\mysync{\{\alpha,\beta\}}$
						$H_1\{\cdot\}$
						$H_2\{\cdot\}$
					]
					$H_3\{\cdot\}$
		 	] 
		 	[.$\mysync{\gamma}$ 
				$H_4\{\cdot\}$
				$H_5\{\cdot\}$
			]  
]
\end{eqnarray*}
The calculation of $\coop{E}{H_1}{\alpha}$ is this: 
\begin{eqnarray*}
\coop{E}{H_1}{\alpha} &=& 
\coop{\ (\  (\  H_1\{\cdot\} \mysync{\{\alpha,\beta\}} H_2\{\cdot\}\  )\ \mysync{\{\theta\}} H_3\{\cdot\} \ \ )}{\ H_1\ }{\ \alpha\ } 
\\ 
& &\ \ \ \ \ \ \cup\ \  \{H_i \mid H_i <^{*}\ (\  H_4\{\cdot\} \mysync{\{\gamma\}} H_5\{\cdot\}\  ) \}
\\
& = & \coop{\  (\  H_1\{\cdot\} \mysync{\{\alpha,\beta\}} H_2\{\cdot\}\  )\ }{\ H_1\ }{\ \alpha\ } 
\\
& &\ \ \ \ \ \ \cup\ \  \{H_4,H_5\}
\\
& = & \coop{\  H_1\{\cdot\} \ }{\ H_1\ }{\ \alpha\ } 
\\
& &\ \ \ \ \ \ \cup \ \{H_i \mid H_i\{\cdot\} <^{*} H_2\{\cdot\}\  \} 
\\
& &\ \ \ \ \ \ \cup\ \  \{H_4,H_5\}
\\
& & \emptyset \ \cup \{H_2,H_4,H_5\} = \{H_2,H_4,H_5\}.
\end{eqnarray*}
Similarly, the calculation of $\coop{E}{H_5}{\alpha}$ is this: 
\begin{eqnarray*}
\coop{E}{H_5}{\alpha} &=& 
\coop{\   (\  H_4\{\cdot\} \mysync{\{\gamma\}} H_5\{\cdot\}\  )\ }{\ H_5\ }{\ \alpha\ } 
\\ 
& &\ \ \ \ \ \ \cup\ \  \{H_i \mid H_i <^{*}\ \Big(\  (\  H_1\{\cdot\} \mysync{\{\alpha,\beta\}} H_2\{\cdot\}\  )\ \mysync{\{\theta\}} H_3\{\cdot\} \ \Big)  \}
\\
& = & \coop{\  H_5\{\cdot\} \ }{\ H_5\ }{\ \alpha\ } 
\\
& &\ \ \ \ \ \ \cup\ \  \{H_1,H_2,H_3\}
\\
& = & \emptyset \ \cup\ \{H_1,H_2,H_3\} = \{H_1,H_2,H_3\}.
\end{eqnarray*}


\end{exmp}

%  explaining the state vector in the context of our grouped pepa models. 
% we need to have a set of vectors for each group.
In the context of large-scale PEPA models, we are often content to abstract from the behaviour of individuals and focus on the evolution of populations \cite{1595779}. In line with this idea, in order to capture the current state of a group $H$, we do not capture the state of each individual instance in that group. Instead, for each local state $C_{x,y}$ in $ds^{*}(H)$, we count how many instances in $H$ exhibit the behaviour associated with $C_{x,y}$. The behaviour of the system is then studied at the level of these populations. 

% the state space representation
% first the idea of \xi(H,C_{x,y}) being a vector
% then the idea of big \xi being a vector of vectors
For a group $H$, let $\xi(H,C_{x,y})$, where $C_x = sc(H)$ and $C_x,y \in ds(C_x)$, represent the number of instances in $H$ which are currently in state $C_{x,y}$. Using this, the vector $\boldsymbol{\xi}(H)$ can be defined as 
\[ \boldsymbol{\xi}(H) = \langle\  \xi(H,C_{x,y}) \ |\ C_{x,y} \in ds^{*}(H)\ \rangle \]
which captures the state of group $H$ at any given time; $\boldsymbol{\xi}(H)$ captures the distribution of the instances in $H$ across the respective local states $ds^{*}(H)$.
Having defined $\boldsymbol{\xi}(H)$ for each group, we can define $\boldsymbol{\xi}$ to be the vector which captures the state of all groups in the model. 
\[\boldsymbol{\xi} = \langle\  \boldsymbol{\xi}(H)\ |\ H \in \group{M}\     \rangle\]
For a PEPA model $\mathbb{M}$ with $N^{h}_{\mathbb{M}}$ groups, each state is represented by a vector $\boldsymbol{\xi}$ consisting of $N^{h}_{\mathbb{M}}$ sub-vectors $\boldsymbol{\xi}_i\ ,\ i \in 1,\ldots, N^{h}_{\mathbb{M}}$.
\begin{eqnarray*}
\boldsymbol\xi & =& \langle \  \boldsymbol\xi(H_1), \boldsymbol\xi(H_2), \ldots, \boldsymbol\xi(H_i), \ldots \boldsymbol\xi(H_{N^{h}_{\mathbb{M}}})\ \rangle \\
\boldsymbol\xi(H_i) & = & \langle \  \xi(H_i,C_{x,1}), \xi(H_i,C_{x,2}), \ldots,  \xi(H_i,C_{x,N_{C_x}})\ \rangle
\end{eqnarray*}
assuming $C_x = sc(H_i)$, $C_x \in \mathcal{C}$,  and the number of local states any $C_x$ instance can experience (i.e. $\# ds(C_x)$ ) is $N_{C_x}$.
The model's dimension, $d_{\mo{M}}$, is defined to be the number of state variables appearing in its state vector.
\[d_{\mo{M}}=\sum_{H\in\group{M}\ ,\ C_x = sc(H)}^{}N_{C_{x}}\]
Each counter $\xi(H,C_{x,y})$ can be regarded as a random variable taking different values as the system evolves and therefore, the state vector, regarded as a vector of random variables. At any given time, a joint probability distribution can be associated with this vector. 

%The state space built by the numerical vectors is more parsimonious and more abstract  
Let $C$ be a local state of a sequential process in $\mathcal{C}_{\mathbb{M}}$ enabling $\mathcal{A}ct(C)$. The apparent rate of an action type $\alpha$ in $C$, denoted by $r_{\alpha}(C)$, is the total rate $C$ offers for one-step $\alpha$ activities. Note that $C$ might be of the following form: 
\[C=(\alpha,r^{\prime}).C^{\prime}+(\alpha,r^{\prime\prime}).C^{\prime\prime} + \ldots\] 
where there is a set of states $C$ can reach via an $\alpha$ activity. 
%\begin{eqnarray*}
%C_{x,y} & \rmdef & (\alpha,r^{\prime}_{\alpha}). C_{x,y^{\prime}} + (\alpha,r^{\prime\prime}_{\alpha}). C_{x,y^{\prime\prime}} + \ldots
%\end{eqnarray*}
%Now consider the transition 
%$C_{x,y} \stackrel{(\alpha,r^{\prime}_\alpha) }{\longrightarrow}C_{x,y^{\prime}}$. For this particular transition, its rate is $r^{\prime}_{\alpha}/r_{\alpha}(C_{x,y})$ where $r_{\alpha}(C_{x,y})$ is defined to be the apparent rate of activity $\alpha$ in the sequential component $C_{x,y}$. In general, the apparent rate of an activity $\alpha$ in a sequential component $C$ can be defined as
$r_{\alpha}(C)$ can be defined as (part of Def. 3.3.1 in \cite{Hillston:1996}):
\begin{eqnarray}
\nonumber r_{\alpha}(C) & =  	\left \{		\begin{array}{ll}
																					r & \ \ \ \ \text{if} \ \ \ \ \  C= (\beta,r).P\  \wedge \  \beta=\alpha \\
																					0 & \ \ \ \ \text{if} \ \ \ \ \  C= (\beta,r).P\  \wedge \  \beta\not=\alpha \\
																					r_{\alpha}(P) + r_{\alpha}(Q) & \ \ \ \ \text{if} \ \ \ \ \  C= P+Q\  \\
																			\end{array} \right. 
\end{eqnarray}
Similarly, we can define $r_{\alpha}(C,C^{\prime})$ to be the apparent rate of an action type $\alpha$ in a sequential component $C$ with respect to those $\alpha$ activities which move $C$ specifically to $C^{\prime}$. 
\begin{eqnarray}
\nonumber r_{\alpha}(C,C^{\prime}) & =  	\left \{		\begin{array}{ll}
																					r & \\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{if} \ \ \ \ \  C= (\beta,r).P\  \wedge \  \beta=\alpha \wedge P = C^{\prime} & \\
																					0 & \\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{if} \ \ \ \ \  C= (\beta,r).P\  \wedge \  ( \beta\not=\alpha\vee P \not= C^{\prime})  & \\
																					r_{\alpha}(P) + r_{\alpha}(Q) & \\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{if} \ \ \ \ \  C= P+Q\  & \\
																			\end{array} \right. 
\end{eqnarray}

The above definitions also support the passive rates. In this paper, we assume that
if a sequential component $C$ is passive with respect to an action type $\alpha$, then, in any $\alpha$ enabling state in $ds(C)$, the activity will have a passive rate.
Moreover, if in a state in $ds(C)$, more than one passive $\alpha$ activities are enabled, then each is given a weight, clarifying the relative probability assigned to each activity. For example, in the process
\[C \rmdef (\alpha,\omega_1 \top).C^{\prime} + (\alpha,\omega_2 \top).C^{\prime\prime}+\ldots\]
$C$ enables two $\alpha$ activities passively. When $C$ performs $\alpha$, with probability $\omega_1/ (\omega_1 + \omega_2)$, it becomes $C^{\prime}$ and with probability $\omega_2/ (\omega_1 + \omega_2)$ it behaves as $C^{\prime\prime}$. 
The rules
\begin{eqnarray} 
\label{eqn:passiveRateRules}
\nonumber1.&& (\omega_1 \top + \omega_2 \top)=(\omega_1 + \omega_2) \top\ \ \ \ \ \ \ \forall \ \  \omega_1,\omega_2 \in \mathbb{N}  \\
2.&& \omega_1 \times (\omega_2 \top) = (\omega_1 \times \omega_2) \top  \\
\nonumber3.&& \top  =  1 \times \top  \\
\nonumber4.&& \min(\omega_1\times\top,\omega_2\times\top) = min(\omega_1,\omega2)\times\top
\end{eqnarray}
are introduced to help calculate the apparent rates for the passive activities. For example, $r_\alpha(C)$ for $C$ above is $(\omega_1 + \omega_2) \top$.

Let us assume that in a group $H_i$ among the instances of the component type $C_x$ ($C_x = sc(H_i)$), some are in state $C_{x,y} \in ds(C_x)$ enabling an activity $\alpha$. Also assume that $\alpha$ is not in $H$'s cooperation set. Undertaking the activity $\alpha$ by any one arbitrary instance causes the number of instances with local state $C_{x,y}$, i.e. $\xi(H,C_{x,y})$ to decrease by one and the number of $C_x$ instances currently in one of the target states ($C_{x,y^{\prime}}$, $C_{x,y^{\prime\prime}}$, \ldots) to increase by one. Therefore, the state of the whole group and the whole model, captured by $\boldsymbol\xi_{i}$ and $\boldsymbol\xi$, will change:
\begin{eqnarray*}
\langle \ \boldsymbol\xi(H_1), \ldots
 ,\boldsymbol\xi(H_i),\ldots, \boldsymbol\xi(H_{N^{h}_{\mathbb{M}}}) \rangle & \stackrel{(\alpha,R_{\alpha}(\boldsymbol\xi(H_i)))}{\xrightarrow{\hspace*{1.05cm}}} & \langle\  \boldsymbol\xi(H_1),\ldots ,\boldsymbol\xi^{\prime}(H_i),\ldots,\boldsymbol\xi(H_{N^{h}_{\mathbb{M}}}) \ \rangle
\end{eqnarray*}
Let us suppose, the state change $C_{x,y} \stackrel{(\alpha,r_{\alpha})}{\longrightarrow} C_{x,y^{\prime}}$ occurs. Then:
\begin{eqnarray*}
\boldsymbol\xi(H_i) & = &  \langle \  \xi(H,C_{x,1}), \ldots, \xi(H,C_{x,y}), \ldots,\xi(H,C_{x,y^{\prime}}),\ldots, \xi(H,C_{N_{C_x}})\ \rangle  \\
\boldsymbol\xi^{\prime}(H_i) & = &  \langle \  \xi(H,C_{x,1}), \ldots, \xi(H,C_{x,y})-1, \ldots, \xi(H,C_{x,y^{\prime}})+1, \ldots \xi(H,C_{N_{C_x}})\ \rangle 
\end{eqnarray*}
For model $\mathbb{M}$, let us define $r^{*}_{\alpha}(H,C,C^{\prime})$, $H\in\mathcal{G}(\mathbb{M})\ ,\ C,C^{\prime} \in ds^{*}(H) $, to denote the apparent rate of action type $\alpha$ in the context of group $H$ with respect to $\alpha$ activities which move instances being in state $C$ specifically to $C^{\prime}$: 
\[ r^{*}_{\alpha}(H,C,C^{\prime}) = \xi(H,C) \times r_{\alpha}(C,C^{\prime})\]
Using this definition, the rate $R_{\alpha}(\boldsymbol\xi(H_i))$ of the transition above is: 
\[ R_{\alpha}(\boldsymbol\xi(H_i)) = \xi(H,C_{x,y}) \times r^{*}_{\alpha}(H_i,C_{x,y},C_{x,y^{\prime}}). \]

We also define $r^{*}_\alpha(H)$ as the apparent rate of the action type $\alpha$ in group $H$ offered by all the instances in that group. Note that in $ds^{*}(H)$, there might be more than one local state enabling $\alpha$.
\[r^{*}_{\alpha}(H) = \sum_{ C \in ds(sc(H)) } \xi(H,C) \times r_{\alpha}(C)\]



%Here, we gradually observed how a transition at the level of a single instance is lifted to the group level. 

Each large-scale model consists of some cooperating groups. Suppose the instances in group $H_i$ which are in state $C_{x,y}$ cooperate with the instances in group $H_j$ who are in state $C_{w,z}$ ($C_{w,z}\in ds(C_w)$, $C_w = sc(H_j)$) on a shared activity of type $\alpha$. 
\begin{eqnarray*}
C_{x,y} \rmdef (\alpha,r_{1}^{\prime}) C_{x,y^{\prime}} + (\alpha,r_{1}^{\prime\prime}) C_{x,y^{\prime\prime}} + \ldots &&\\  
C_{w,z} \rmdef (\alpha,r_{2}^{\prime}) C_{w,z^{\prime}}+ (\alpha,r_{2}^{\prime\prime})  C_{w,z^{\prime\prime}} +\ldots&&
\end{eqnarray*}

Undertaking $\alpha$ by two arbitrary $C_{x,y}$ and $C_{w,z}$ instances (one of each) and becoming respectively, $C_{x,y^{\prime}}$ and $C_{w,z^{\prime}}$,  will change both $\boldsymbol\xi(H_i)$ and $\boldsymbol\xi(H_{j})$; 
$\boldsymbol\xi  \stackrel{(\alpha,R_{\alpha}(\boldsymbol\xi(H_i),\boldsymbol\xi(H_j)))}{\xrightarrow{\hspace*{2.55cm}}} \boldsymbol\xi^\prime$ where:
\begin{eqnarray*}
\boldsymbol{\xi} &=& \langle \ \boldsymbol\xi(H_1), \ldots
 ,\boldsymbol\xi(H_i),\ldots,\boldsymbol\xi(H_j),\ldots, \boldsymbol\xi(H_{N^{h}_{\mathbb{M}}}) \rangle  \\ 
\boldsymbol{\xi}^{\prime} & = & \langle\  \boldsymbol\xi(H_1),\ldots ,\boldsymbol\xi^{\prime}(H_i),\ldots,\boldsymbol\xi^{\prime}(H_j),\ldots,\boldsymbol\xi(H_{N^{h}_{\mathbb{M}}}) \ \rangle \\
\boldsymbol\xi^{\prime}(H_i) & = &  \langle \  \xi(H,C_{x,1}), \ldots, \xi(H,C_{x,y})-1, \ldots, \xi(H,C_{x,y^{\prime}})+1, \ldots \xi(H,C_{N_{C_x}})\ \rangle  \\
\boldsymbol\xi^{\prime}(H_j) & = &  \langle \  \xi(H,C_{w,1}), \ldots, \xi(H,C_{w,z})-1, \ldots, \xi(H,C_{w,z^{\prime}})+1, \ldots \xi(H,C_{N_{C_w}})\ \rangle 
\end{eqnarray*}
The rate at which the above transition is observed depends on the states of both $H_i$ and $H_j$.
According to PEPA's semantics; it can be calculated as follows: 
\begin{eqnarray*}
R_{\alpha}(\boldsymbol\xi(H_i),\boldsymbol\xi(H_j)) = \frac
{r^{*}_{\alpha}(H_i,C_{x,y},C_{x,y^{\prime}})}
{r^{*}_{\alpha}(H_i)}
\frac
{{r^{*}_{\alpha}(H_j,C_{w,z},C_{w,z^{\prime}})}}
{r^{*}_{\alpha}(H_j)} 
\min({r^{*}_{\alpha}(H_i)},{r^{*}_{\alpha}(H_j)})
\end{eqnarray*}


%\begin{eqnarray*}
%\boldsymbol\xi & = &  \langle \  \boldsymbol\xi_{1}, \boldsymbol\xi_{2}, \ldots, \boldsymbol\xi_{i}, \ldots, \boldsymbol\xi_{j}, \ldots, \boldsymbol\xi_{N_{\mathbb{M}}}\ \rangle  \\
%\boldsymbol\xi^{\prime} & = &  \langle \  \boldsymbol\xi_{1}, \boldsymbol\xi_{2}, \ldots, \boldsymbol\xi_{i}^{\prime}, \ldots, \boldsymbol\xi_{j}\prime, \ldots, \boldsymbol\xi_{N_{\mathbb{M}}}\ \rangle  \\ \\
%\boldsymbol\xi_{i} & = & \langle\  \xi_{i,1}, \ldots, \xi_{i,y},\ldots,\xi_{i,y^{\prime}},\ldots, \xi_{i,n_x}\ \rangle \\
%\boldsymbol\xi_{j} & = & \langle\  \xi_{j,1}, \ldots, \xi_{j,y},\ldots,\xi_{j,z^{\prime}},\ldots, \xi_{j,n_w}\ \rangle \\ \\
%\boldsymbol\xi_{i}^{\prime} & = & \langle\  \xi_{i,1}, \ldots, \xi_{i,y}-1,\ldots,\xi_{i,y^{\prime}}+1,\ldots, \xi_{i,n_x}\ \rangle \\
%\boldsymbol\xi_{j} & = & \langle\  \xi_{j,1}, \ldots, \xi_{j,z}-1,\ldots,\xi_{j,z^{\prime}},+1 \ldots, \xi_{j,n_w}\ \rangle
%\end{eqnarray*}
%According to \cite{scalable,Hayden:2010}, which provide the way for calculating the rates at the level of cooperating groups, $R_{\alpha}$ can be calculated as follows:  
%\begin{eqnarray*}
%\lefteqn{R_{\alpha} = } \\ 
%&& \frac{\xi_{i,y} r_{\alpha}(C_{x,y},C_{x,y^{\prime}}) }{r_{\alpha}(H_i)} \frac{\xi_{j,z} r_{\alpha}(C_{w,z},C_{w,z^{\prime}})}{r_{\alpha}(H_j)} min(r_\alpha(H_i),r_\alpha(H_j))
%\end{eqnarray*}

%According to \cite{scalable}, this rate can be calculated as:
%$r_\alpha(\xi) = r_\alpha(\xi_i) = \xi_{i,j} r_{\alpha}(C_{i,j})$ where $r_{\alpha}(C_{i,j})$, $C_{i,j} \in d_s(C_i)$ denotes the rate defined for activity $\alpha$ in an instance being in state $C_{i,j}$. 

%The \emph{apparent} rate of an activity with respect to the instances of component type $C_i$  can be defined as: $r^{*}_{\alpha}(C_i)=\sum_{j=1}^{n_i}r_\alpha(C_{i,j})\times \xi_{i,j}$; this is the rate at which the activity $\alpha$ will be undertaken considering the whole population of the instances of component type $C_i$. As an example, consider activity $(log,r_l)$ in the component type $Server$. Given that the system's state is captured by the vector 
%\[\xi = \langle \xi_{Server_{idle}}, \xi_{Server_{logging}},\xi_{Server_{broken}},\xi_{Client_{requesting}},\xi_{Client_{thinking}}\rangle\]
%then the rate of this activity is $r_{log}(\xi) = r_{log} \times \xi_{Server_{logging}}$ and upon firing, it takes the system into the state 
%\[\xi_{Server}=\langle \xi_{Server_{idle}}+1, \xi_{Server_{logging}}-1,\xi_{Server_{broken}},\xi_{Client_{requesting}},\xi_{Client_{thinking}}\rangle. \]

%For activities which are shared between the instances of different component types, there is a similar approach for lifting the transitions to the population level. Assume that the instances of component type $C_i$ who are in state $C_{i,j}$ and instances of component type $C_k$ who are in state $C_{k,l}$ cooperate on a shared activity $(\alpha,r_\alpha)$. Then, the following transition would be possible: 
%Now consider $\tau^{\prime}$ and assume that it is a shared activity between the instances of component type $C_i$ who are in state $C_{i,j}$ and instances of component type $C_k$ who are in state $C_{k,l}$:
%\begin{eqnarray*}
%\begin{inference}
%{C_{i,j} \stackrel{(\tau^{\prime},r_{\tau^{\prime}}(C_{i,j}))}{\longrightarrow} C_{i,j^{\prime}} \ \ \ \ \ \bigwedge \ \ \ \ \
%{C_{k,l} \stackrel{(\tau^{\prime},r_{\tau^{\prime}}(C_{k,l}))}{\longrightarrow} C_{k,l^{\prime}}}}
%{ C_{i,j} \mysync{L} C_{k,l} \stackrel{(\tau^{\prime},min(      r_{\tau^{\prime}}(C_{i,j}),r_{\tau^{\prime}}(C_{k,l}))                     )}{\longrightarrow} C_{i,j^{\prime}} \mysync{L} C_{k,l^{\prime}}}
%\end{inference}
%\end{eqnarray*}
%
%Let us now consider the transition of the type $\tau^{\prime}$ at the population level. The sub-vectors capturing specifically the states of the instances of the component types $C_i$ and $C_k$ are $\xi_i$ and $\xi_{k}$ respectively. When an instance of a transition $\tau^{\prime}$ fires, both population sub-vectors change and as the result, the state of the whole system also changes: 
%\begin{eqnarray*}
%\begin{array}{l}
%\langle 
%\xi_{1,1}, , \ldots, \xi_{1,n_1},\ldots \\
%\xi_{i,1}, , \ldots\, \xi_{i,j}, \ldots, \xi_{i,j^{\prime}} , \ldots, 	\xi_{i,n_i}, \ldots \\
%\xi_{k,1}, , \ldots\, \xi_{k,l}, \ldots, \xi_{k,l^{\prime}} , \ldots, 	\xi_{k,n_k}, \ldots \\
%\xi_{i,j^{\prime}} , \ldots, 	\xi_{i,n_i} 
%\rangle
%\end{array} 
%\stackrel{(\alpha,R_{\alpha})}{\rightarrow}
%\begin{array}{l}
%\langle 
%\xi_{1,1}, , \ldots, \xi_{1,n_1},\ldots  \\
%\xi_{i,1}, , \ldots\, \xi_{i,j}-1, \ldots, \xi_{i,j^{\prime}}+1 , \ldots, 	\xi_{i,n_i}, \ldots  \\
%\xi_{k,1}, , \ldots\, \xi_{k,l}-1, \ldots, \xi_{k,l^{\prime}}+1 , \ldots, 	\xi_{k,n_k}, \ldots \\
%\xi_{i,j^{\prime}} , \ldots, 	\xi_{i,n_i} 
%\rangle
%\end{array} && 
%\end{eqnarray*}
%$R_{\alpha}$, the rate of this transition, is a function of two sub-vectors $\xi_i$ and $\xi_{k}$: 
%
%
%For the detailed calculations, please refer to \cite{scalable}.
%


==> RelatedWork/relatedWork.tex <==
\section{Related Work} 
\label{relatedWork}

In the context of modelling large-scale stochastic systems, regardless of the notation used for specifying the model (process algebra, Petri-net, queueing networks), 
%i.e. whether it is specified using queueing networks, stochastic Petri-Nets or a stochastic process algebra such as PEPA, 
both the construction of the model's complete CTMC and the derivation of its joint probability distribution in full, are computationally expensive or infeasible. 
In such situations, it is common practise to use an aggregation or a decomposition method which provides a reduced size CTMC to work with or use methods which, instead of calculating the full distributions, produce some marginal ones. 
These simplifying methods usually exploit the structure of the model's CTMC and allow for a timely analysis which otherwise would have been impossible. 
%The abstract CMTCs are usually constructed directly from the model description and building the model's whole state space is avoided.
%The concept of exploiting the structure of a CTMC in order to reduce its analysis cost and  replacing the computation of the full joint probability distribution with the computation of one or more marginal probability distributions is commonly used in different modelling formalisms, such as queueing networks, stochastic Petri-Nets or stochastic process algebra.  
Our aggregation method follows the same idea and therefore, it can conceptually be related to two existing techniques: the idea of ``quasi-separability'' and the method of ``lumpability''.

The technique of quasi-separability was originally developed by Mitrani and Wright for queueing networks \cite{Mitrani1994151} and in \cite{Thomas1998,thomas1999extending}, Thomas and Gilmore extended the technique for applying on Markovian process algebra models. 
Given a process, the modeller categorises each constituent component as being either an \emph{environment} component or an \emph{internal} one. 
The environment components are assumed to control the model's high level mode of operation and the internal components capture the internal state.
If the model satisfies a so called \emph{quasi-separability condition}, then from the model, a number of sub-models are generated where each sub-model captures the dynamics of some internal components in combination with all environment ones. 
The idea is that for the internal components which fall in a sub-model, their dynamics is independent of the other internal ones and therefore, their behaviour can be studied \emph{in separation} by considering only their own sub-model. 
Using this method, for a given model, instead of getting the probability distribution on all the model's components, for each sub-model, one marginal distribution is derived. 
Our work is in line with \cite{Mitrani1994151,Thomas1998,thomas1999extending}. Here, we have extended the applicability of the method and proposed the foundations for using it on process algebra population models. 
In particular, for a large-scale model in which there is an interaction between small and large groups, we established the conditions which determine whether the small groups can be separated from the rest of the model and their dynamics be studied independently. 

The second method related to ours is lumpability\footnote{The type of lumpability we refer to is \emph{ordinary lumpability} defined in \cite{p1994} and illustrated also in \cite{Hillston:1996}, Section 5.}. 
For a given model, this method first tries to form a partition on the model's CTMC in a way that the partition satisfies the \emph{lumpability} condition. 
If successful, it then generated the model's aggregated CTMC in which each partition is represented by a single state. 
The size of the aggregated CTMC is smaller than the original one and therefore, it provides the means for efficient performance analysis. 
Essentially, our method follows the same approach. 
For a model which satisfies the aggregation conditions, its aggregated CTMC is constructed and used for further performance studies. 
However, it is important to note that our conditions are less stringent than those for lumpability, and will aggregate a larger class of models. 
More specifically, for a given model in our sub-class, the presence of boundary states in its state space might be completely detrimential for the the lumpability method to be able to generate its CTMC where as in such situations, our aggregation method can operate and generate the model's aggregated CTMC.
% backup for chapter. 
%The technique of quasi-separability was originally developed for queueing networks \cite{Mitrani1994151}. In \cite{Thomas1998,thomas1999extending}, Thomas and Gilmore developed the following process for applying the technique on models specified in Markovian process algebra such as PEPA. Given a PEPA model, the components in its system equation are divided in two categories; components which capture the system's high-level operation state (called \emph{environment} components) and the components which capture the internal state. At this stage, the following two conditions are checked on the model: a) there is no interaction between any two internal components and, b) for any interaction taking place between an internal component and an environment component, the rate of the interaction is controlled by the latter. The authors show that if the model satisfies these conditions, then, using the model, for each internal component a dedicated sub-model can be constructed from which the component's marginal probability distribution can be calculated. The marginal distribution for a component expresses the probability of the component being in different states it can exhibit. The state space calculated for an internal component $comp_i$ captures the evolution of that internal component and its interactions with the set of model's environment components. Such a sub-model abstracts away from the changes on the other internal variables. In essence, for the model which satisfies the conditions, the internal components can be analysed \emph{in separation}. 

%In the context of our method, given a PEPA model, the modeller first specifies which populations are small and which are large. In the next step, we check if the interactions between the small populations and large ones are completely controlled by the small populations. If this condition holds, then, our aggregation method is used to construct an aggregate CTMC which captures the dynamics of the small populations. This aggregate CTMC is built, having ignored the interactions the small populations have with the large ones. The idea here is that for a conforming model, the dynamics of its small populations can be safely separated from the rest of the model and their evolution can easily be studied in isolation. Our approach is similar to \cite{Thomas1998,thomas1999extending} also in the sense that the conditions we check are similar. 

%Note, however, that our goal is distinct from  \cite{Thomas1998,thomas1999extending}. Here, we aim to show that although the complete CTMC of the model, due to the presence of very large populations, is computationally expensive to build and analyse, nevertheless if the model satisfies some conditions, then an aggregation scheme is feasible and therefore, dynamics of the small populations can be efficiently studied. The separation of the small populations from the model is a consequence of the aggregation method proposed. 

%This method aims at reducing the size of the CTMC and therefore, constructing a more abstract CTMC for which the analysis is computationally less expensive. Given a CTMC, the method tries to form a partition of its set of states in a way that for any two partitions $t_i$, $t_j$ the following condition holds: 
%\[\sum_{ m \in t_j } q(n,m) = \sum_{m \in t_j} q(n^{\prime},m). \]
%where $n$ and $n^{\prime}$ are two arbitrary states in partition $t_i$ and $q(n,m)$ is the rate of the transition going from the state $n$ in partition $t_i$ to the other state $m$ in partition $t_j$. If such a partition exists, then, using the initial complete CTMC, one builds a more compact CTMC where for each partition in the former, one state is constructed in the latter. A state in the lumped CTMC represents all the states of the first CTMC which belong to one partition. 

%Our method follows the same approach. Essentially, for a PEPA model which satisfies condition 1, 2, using solely the model, our method first identifies each group of states which can be represented by one aggregate state. Then, it directly constructs a compact CTMC which consists only of the aggregate states. Hence, informally, the similarity between our method and the lumpability is that both lead to aggregated CTMCs. However, note that, formally, our condition are less stringent than those for ordinary lumpability, and will aggregate a larger class of models. 
%the lumpability method, when given a conforming model's complete CTMC, is not capable of finding the aggregate CTMC which our method finds for the same model; our conditions are less stringent than those. 
%This can be easily shown by the following example. Consider the state space of Fig. \ref{fig:fullstatesapce}. Fig. \ref{X} shows the aggregate CTMC generated by our method. Our method will assign the states 1,2,3 to the same group as the state of the servers in those states are identical. However, lumpability does not make the same grouping because in each of the states 2 and 3 there are $req$ transitions into the states 6 and 7 of group 2, whereas there is no such a transition into any of the states of the group 2 from state 1. Hence, the partitioning induced by our method is not a lumpable partition. Therefore, our aggregation method needs to be distinguished from the 

==> pepaSOS.tex <==
\begin{figure}[ht!]
\centering
\begin{tabular}{|l|}
\hline
%\\
{\bf~~~Prefix} \\
\begin{minipage}[c]{13.0cm}
\begin{center}
$ {\displaystyle
     \frac{}
     {(\alpha,r).E \stackrel{(\alpha,r)}{\vlra} E} }$  
\end{center} \end{minipage}
%% \ \
%% \begin{minipage}[c]{6.5cm}
%% \begin{center}
%% $ {\displaystyle \left(
%%     \frac{}
%%  {((\alpha,r).E, t) \stackrel{(\alpha,r)}{\vlra} (E, t + \Delta
%%  t)}\right)}$   
%% \end{center}
%% \end{minipage} \\ 
\\
{\bf~~~Cooperation} 
\\
\begin{minipage}[c]{6.5cm}
\begin{center}
$ {\displaystyle
     \frac{E \stackrel{(\alpha,r)}{\vlra} E'}
          {E\mysync{\:L}\;F \stackrel{(\alpha,r)}{\vlra} E'\mysync{\:L}\;F} \; 
                                                          (\alpha \notin L)}$
\end{center}
\end{minipage}
\ \
\begin{minipage}[c]{6.5cm} 
\begin{center}
$ {\displaystyle
     \frac{F \stackrel{(\alpha,r)}{\vlra}F'}
          {E\mysync{\:L}\;F \stackrel{(\alpha,r)}{\vlra} E\mysync{\:L}\;F'} \; 
                                                           (\alpha \notin L)}$ 
\end{center}
\end{minipage} \\ \\ 

\begin{minipage}{14.0cm}
\begin{center}
$ {\displaystyle
   \frac{E \stackrel{(\alpha,r_1)}{\vlra} E'\;\;
                                       F \stackrel{(\alpha,r_2)}{\vlra} F'}
        {E\mysync{\:L}\;F \stackrel{(\alpha,R)}{\vlra} E'\mysync{\:L}\;F'}     \;
            (\alpha \in L)}$ \hspace{0.5cm} \mbox{where } 
                ${\displaystyle  R = \frac{r_1}{r_{\alpha}(E)} \frac{r_2}
                         {r_{\alpha}(F)} \min(r_{\alpha}(E),r_{\alpha}(F))}$ 
%                ${\displaystyle  R = \frac{r_1}{q(E, \alpha)} \frac{r_2}
%                         {q(F, \alpha)} \min(q(E, \alpha),q(F,\alpha))}$
\end{center}
{\small \mbox{} \hspace{8.0cm} $r_{\alpha}(E)$: the apparent rate of $\alpha$ in $E$}   
\end{minipage}
% \\ 
\\
{\bf~~~Choice} 
\\
\begin{minipage}[c]{6.5cm}
\begin{center}
${\displaystyle
  \frac{E \stackrel{(\alpha,r)}{\vlra} E'}
                          {E + F \stackrel{(\alpha, r)}{\vlra}E'}}$
\end{center}
\end{minipage}
\  \
\begin{minipage}[c]{6.5cm}
\begin{center}
${\displaystyle
    \frac{F \stackrel{(\alpha,r)}{\vlra} F'}
                                   {E + F \stackrel{(\alpha,r)}{\vlra}F'}}$
\end{center}
\end{minipage} \\ 
 
\\
{\bf~~~Constant} 
\\
\begin{minipage}{13.0cm}

\begin{center}
$ {\displaystyle
     \frac{E \stackrel{(\alpha,r)}{\lra}E'}{A\stackrel{(\alpha,r)}{\lra} 
                                                        E'} \; (A \rmdef E)}$ 
\end{center}
\end{minipage} \\ \\
\hline
\end{tabular}
\caption{structured operational semantics of PEPA}
\label{fig:pepaSOS}
\end{figure}
